Achieving Performance and Safety in Large Scale Systems with Saturation using a Nonlinear System Level Synthesis Approach

We present a novel class of nonlinear controllers that interpolates among differently behaving linear controllers as a case study for recently proposed Linear and Nonlinear System Level Synthesis framework. The structure of the nonlinear controller allows for simultaneously satisfying performance and safety objectives defined for small- and large-disturbance regimes. The proposed controller is distributed, handles delays, sparse actuation, and localizes disturbances. We show our nonlinear controller always outperforms its linear counterpart for constrained LQR problems. We further demonstrate the anti-windup property of an augmented control strategy based on the proposed controller for saturated systems via simulation.

==> [ACC2020] Saturation_Arxiv_ver/blend_v1.tex <==
% \subsection{LTI System Level Approach}
% \noindent For a linear system $$ x_{t+1} =  Ax_t + B u_t + w_t, $$
% \cite{slsacc} has shown that for any matrices $R_k, M_k$ that satisfy the affine constraints
% \begin{subequations}
% \label{eq:lin-feaibility}
% \begin{align}
%     R_{1} &= I \\
%     R_{k+1} &= A R_k + B M_k, \quad k\leq T-1 \\
%     0 &= A R_T + B M_T, 
% \end{align}
% \end{subequations}

%\todo[inline]{Ideally the above Intro starts from linear sls and says that we have this relationship between closed loop maps and realizing controllers.. Then just say that we have way to extend this realtionship for general causal systems (ref to other paper)...and then say that here we will only focus on a particular type of nonlinear extension that helps for large-scale linear saturated systems }

%\subsection{Nonlinear SLS for Linear Input-Saturated System}
%\noindent Consider the linear system with input saturation
%\begin{align}\label{eq:linsat}
%    x_{k+1} = Ax_k + B \mathbf{Sat}(u_k) + w_k
%\end{align}
%We are proposing the following system level controller implementation 
%\begin{subequations}
%\begin{align}
%\label{eq:nl-controller-1}
%    \hat{w}_t &= x_t - \sum^{N}_{i=1}\sum^{T-1}_{k=1}R^{i}_{k+1}G^i(\hat{w}_{t-k})\\
%    \label{eq:nl-controller-2} u_t &= \sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(\hat{w}_{t-k})
%\end{align}
%\end{subequations}
%parametrized by matrices $R^i_k$ and $M^i_k$ that satisfy:
%%\begin{subequations}
%%\label{eq:lin-feaibility}
%%\begin{align}
%%    R^i_{1} &= I \\
%%    R^i_{k+1} &= A R^i_k + B M^i_k, \quad k\leq T-1 \\
%%    0 &= A R^i_{T} + B M^i_{T}, 
%%\end{align}
%%\end{subequations}
%and some nonlinear maps $G^{i}$. A crucial design principle will be that the maps $G^{i}$ are chosen such that the controller never enters the saturated regime:
%\begin{asp}\label{asp:G}
%Assume $G^{i}( \cdot )$ are chosen such that for all $z_1$, $\dots$, $z_T$ holds:
%$$\mathbf{Sat}\left(\sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(z_k)\right) = \sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(z_k)$$
%\end{asp}
%Now, given our design assumption \aspref{asp:G} substituting the dynamics \eqref{eq:linsat} in \eqref{eq:nl-controller-1} and then using the same expressions \eqref{eq:nl-controller-1}, \eqref{eq:nl-controller-2} to express $x_{t-1}$ and $u_{t-1}$ in terms of  $\hat{w}_{t-k}$, $1 \leq k \leq T$, we get the following equation for the dynamics of $\hat{w}_t$:
%\begin{align}
%   \hat{w}_{t+1} &= A(\hat{w}_t - \sum^{N}_{i=1} G^i(\hat{w}_{t})) + w_{t}
%\end{align}
%We will refer to the internal state $\hat{w}_t$ as the \textit{effective disturbance}. If we have stability for $\hat{w}_t$, the relation \eqref{eq:nl-controller-1} and \eqref{eq:nl-controller-2} show that we also imply stability for the state $x$ and input $u$, since 
%\begin{align*}
%    x_t &= \hat{w}_t + \sum^{N}_{i=1}\sum^{T-1}_{k=1}R^{i}_{k+1}G^i(\hat{w}_{t-k})\\ u_t &= \sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(\hat{w}_{t-k})
%\end{align*}
%
%For this paper we will choose 
%\begin{align}
%    G^i(w) = \p{i}{w}-\p{i-1}{w}
%\end{align}
% where $\p{i}{w}$ denote different projection operators. Correspondingly, the dynamics of  \eqref{eq:intDyn} then become 
% \begin{align}
%     \label{eq:intDyn2}
%   \hat{w}_{t+1} &= A(\hat{w}_t - \p{N}{\hat{w}_t}) + w_{t}
% \end{align}

As introduced in the previous section, system level controllers defined in \defref{def:SL} can implement arbitrary CLM for causal nonlinear systems of the form \eqref{eq:sys}. The results in \cite{NLSLSHODoyle2019} motivate a new approach for nonlinear control synthesis: Searching for stable operators $\TX$, $\TU$ that are CLMs satisfying \eqref{eq:feasnl} and constructing a corresponding system level controller $\SL{\TX}{\TU}$ by \defref{def:SL}.

It is conceivable that the generality of this approach could lead to an entirely new direction of nonlinear dynamic control methods. Serving as a first step towards exploring the potential of this new perspective, the remainder of this paper focuses on a subset of nonlinear system level controllers $\SL{\TX}{\TU}$ that proves particularly useful for controlling large-scale linear systems subject to state/input constraints and input saturation.

%In particular we will restrict ourselves to the class of controllers $\SL{\TX}{\TU}$ where $\TX$ and $\TU$ are structured as
%
%Here $G^{i}, i\in \set{N}$ are to-be-designed nonlinear functions.  $R^{(i)}_k \in \RR^{n\times n}$, $M^{(i)}_k \in \RR^{p\times n}$ are matrices associated with linear FIR CLM $\CLM{x,i}$,$\CLM{u,i}$, $i \in \set{N}$ of horizon $T$ for a linear system of interests: 
%\begin{align} \label{eq:syslin}x_{k+1} =Ax_k + Bu_k + w_k \end{align}
%such that for each $i \in \set{N}$, $\CLM{x,i}$,$\CLM{u,i}$ satisfies \eqref{eq:lin-feaibility}.  The dynamic controller \eqref{eq:SLeq} that achieves \eqref{eq:n-blend} has the following explicit form:
%\begin{subequations}
%	\begin{align}
%	\label{eq:nl-controller-1}
%	\hat{w}_t &= x_t - \sum^{N}_{i=1}\sum^{T-1}_{k=1}R^{i}_{k+1}G^i(\hat{w}_{t-k})\\
%	\label{eq:nl-controller-2} u_t &= \sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(\hat{w}_{t-k}).
%	\end{align}
%\end{subequations}
%\todo[inline]{The internal dynamics part is missing... you say the dynamic controller achieves the CLMs but that's not true, because if you don't choose $\Sigma_i G^i = I$, then 14a and 14b are not realizable CLM's only approximate ones..}


In particular we will restrict ourselves to the class of controllers $\SL{\TX}{\TU}$ where $\TX$ and $\TU$ are structured as
\begin{subequations}
	\label{eq:n-blend}
	\begin{align}
	% \clm{x}{t}(w_{t-1:t-T}) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}R^{(i)}_{k} (\p{i}{w_{t-k}}-\p{i-1}{w_{t-k}} )\\
	\clm{x}{t}(\cdot) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}R^{(i)}_{k}  (\p{i}{w}-\p{i-1}{w})\\
	\clm{u}{t}(\cdot) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}M^{(i)}_{k}( \p{i}{w}-\p{i-1}{w}).
	\end{align}
\end{subequations}

We choose $\eta_N\geq\eta_{N-1}\geq \dots \geq \eta_0 =  0$ and  the operator $\p{i}{\cdot}:\RR^{n} \rightarrow \RR^n$ as any nonlinear function with a projection-like property defined for parameter $\eta_i$. $R^{(i)}_k \in \RR^{n\times n}$, $M^{(i)}_k \in \RR^{p\times n}$ are matrices associated with linear FIR CLMs $\CLM{x,i}$,$\CLM{u,i}$, $i \in \set{N}$ of horizon $T$ for a linear system of interests: 
\begin{align} \label{eq:syslin}x_{k+1} =Ax_k + Bu_k + w_k \end{align}
with $x_t \in \RR^n$,$w_t \in \RR^n$, $u \in \RR^p$ such that for each $i \in \set{N}$, $\CLM{x,i}$,$\CLM{u,i}$ satisfies \eqref{eq:lin-feaibility}.
 Concretely, we consider two specific nonlinear projections:
 
 \begin{defn}[Saturation Projection]\label{def:sat}
 	Let vector $w = [w^1, \dots, w^n]^T$. The saturation projection is an element-wise projection:\begin{align}
 	\p{}{w}:= \begin{bmatrix}
 	\sat(w^1,\eta)\\ \vdots\\
 		\sat(w^n,\eta)
 	\end{bmatrix}
 	\end{align}
 	where $\sat(w,\eta) = \text{sign}(w) \max\{|w|,\eta\}$.
 \end{defn}

\begin{defn}[Radial Projection] \label{def:radial}
The radial projection is defined as:\begin{align}
    \p{}{w}:= \frac{\sat(\|w\|_{\infty}/\eta,1)}{\|w\|_{\infty}/\eta} w
\end{align}
\end{defn}


Unless otherwise specified, the results derived in the rest of the paper hold for both projections.
%\begin{rem}
% For $n=1$, radial projection and saturation projection coincide with each other. The radial and saturation projection operator act as the identity whenever $\|w\|_{\infty} \leq \eta$. Otherwise, the radial projection rescales $w$ such that $\|\p{}{w}\|_{\infty} = \eta$ whereas the saturation projection performs element-wise radial projection.
%\end{rem}


The proposed nonlinear controller $\SL{\CLM{x}}{\CLM{u}}$ can be thought of as a \textit{nonlinear blend} of the \textit{linear} FIR controllers $\SL{\CLM{x,i}}{\CLM{u,i}}$, $i \in \set{N}$. Although the nonlinear operator $\CLM{x}$, $\CLM{u}$ differs from its linear components $\CLM{x,i}$, $\CLM{u,i}$ only by the static nonlinear function $\p{i}{w}$, the upcoming sections will demonstrate that this simple additional nonlinearity proves surprisingly useful. In particular, $\eta_i$'s separate any disturbance $w_t$ into $N$ zones such that for each $i$th linear controller $\SL{\CLM{x,i}}{\CLM{u,i}}$, only the portion of $w_t$ that "falls" between $\eta_i$ and $\eta_{i-1}$ is acted upon. Intuitively, one could choose different behaviours for various portions of the disturbance signal, specifying either performance or safety properties.





For ease of exposition, we focus on the two-zone case of the proposed controller $\SL{\CLM{x}}{\CLM{u}}$ though all the analysis extends naturally to the $N$-zone case. 
Thus, \eqref{eq:n-blend} simplifies to
\begin{align}
    \clm{x}{t}(w_{t-1:0}) = \sum^{\min\{T,t\}}_{k=1} &\R1{k} \p{1}{w_{t-k}} + \label{eq:NL-map}\\
    & \R2{k}(\p2{w_{t-k}} - \p1{w_{t-k}}) \nonumber \\
    \clm{u}{t}(w_{t-1:0}) = \sum^{\min\{T,t\}}_{k=1} &\M1{k} \p{1}{w_{t-k}} +\nonumber \\
    & \M2{k}(\p2{w_{t-k}} - \p1{w_{t-k}}). \nonumber\label{eq:NL-map-2}
\end{align}
% The operators $\TX$, $\TU$ are nonlinear due to the nonlinearity introduced by the projection $\p{}{w}$. Nevertheless, by plugging equation \eqref{eq:NL-map} into the general CLM conditions of \thmref{thm:sufnec}, it can be verified that $\TX$, $\TU$ are nonlinear CLMs of the linear system \eqref{eq:syslin} for small disturbances. This is summarized in the next lemma:
% \begin{lem}
% If $\{\CLM{x,i}$,$\CLM{u,i}\}_{i = 1,2}$ are CLM for \eqref{eq:syslin}, then the nonlinear operators $\TX$, $\TU$ defined in \eqref{eq:NL-map} are CLMs of \eqref{eq:syslin} for all $\b{w}$ that satisfy $\sup_k \|w_k\|_{\infty} \leq \eta_2$.
% \end{lem}
Note that system level controller $\SL{\CLM{x}}{\CLM{u}}$ of the two-zone CLM is internally stabilizing and achieves the two-zone CLM behaviour for \eqref{eq:syslin}  as long as $\|\b{w}\|_{\infty} \leq \eta_2$ with $x_0 = 0$. 
% The closed loop dynamics simplify to:
% \begin{subequations}
% \label{eq:cleq_blend}
% \begin{align}
%   \label{eq:clint_blend} 
%   \hat{w}_{t+1} &= A(\hat{w}_t-\p{2}{\hat{w}_t}) + w_t\\
%     \label{eq:clx_blend}    
%     x_t &= \Tx{t}\left(0,0,\hat{w}_{t-1:1}\right)+\hat{w}_{t}\\
%     \label{eq:clu_blend}u_t &= \Tu{t}\left(0,\hat{w}_{t:1}\right)
% \end{align}
% \end{subequations}

% \begin{rem}
% The blending of \textit{two} linear CLM in \eqref{eq:NL-map} can be naturally extended to \textit{$N$} linear CLM by extending \eqref{eq:NL-map} to the form:
% \begin{align}\label{eq:blend}
% \clm{x}{t}(w_{t-1:t-T}) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}R^{(i)}_{k} \p{i}{w_{t-k}} \\
% \clm{u}{t}(w_{t-1:t-T}) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}R^{(i)}_{k} \p{i}{w_{t-k}} 
% \end{align}
% where $R^{(i)}_{k}$, $M^{(i)}_{k}$ are matrices associated with $N$ linear FIR CLM $\CLM{x,i}$, $\CLM{u,i}$.
% \end{rem}

In the remainder of this paper we will explore the consequence of this blending technique for decentralized control design with respect to input saturation and state constraints in linear systems. It will become clear that with the simple projection nonlinearity, \eqref{eq:NL-map} offers a variety of advantages over linear controllers.

==> [ACC2020] Saturation_Arxiv_ver/intro_v1.tex <==


In this paper, we propose a novel offline distributed nonlinear controller synthesis procedure that outperforms any optimal linear controller for constrained LQR problem \cite{maciejowski2002predictive, zhang2013distributed,li2011disturbance,SLSChenAnderson2019}. In addition, the same controller inherently prevents windup-instabilities in saturated linear systems which are traditionally mitigated via additional anti-windup design \cite{kothare1994unified, kolmanovsky2014reference,hu2008anti}. Another significant advantage of the approach, is that despite being a nonlinear synthesis method it naturally enjoys the same benefits as the linear system level approach introduced in \cite{anderson2019system}, which makes it scalable in the large-system setting. 

 Our work is largely based on \cite{NLSLSHODoyle2019}, which describes the system-level characterization of closed loops of general nonlinear discrete-time systems. Moreover, \cite{NLSLSHODoyle2019} introduces a simple universal control structure, called a system level controller, that has the capacity to stabilize any nonlinear system if parametrized with the according closed loop maps. In this paper, we will show that just using a very special case of the framework presented in \cite{NLSLSHODoyle2019} provides new promising tools for control design. In particular, we will illustrate how a simple projection nonlinearity can become a powerful tool for solving the problems described above. 

 
The rest of the paper starts with a review on nonlinear System Level Synthesis (NLSLS) in \secref{sec:nlsls}. The proposed nonlinear controller is introduced in \secref{sec:blend}, followed by \secref{sec:lqr} where the constrained LQR problem is discussed. We show in \secref{sec:ls} that the proposed nonlinear controller has natural anti-windup properties and therefore allow for large-scale distributed design. Numerical simulation in \secref{sec:sim} validates the presented theory. 

==> [ACC2020] Saturation_Arxiv_ver/lqr_v1.tex <==
We present a novel nonlinear controller synthesis procedure for a class of constrained LQR problems using the proposed SL controller with CLMs \eqref{eq:NL-map}. In particular, we will show that the synthesized  nonlinear blending system level controller is guaranteed to outperform any linear controller for the class of constrained LQR problems to be discussed. Additionally, we comment on how structural constraints for large-scale systems such as delay, actuation sparsity, and localization can be easily accommodated for our nonlinear controller. 

\subsection{Problem Statement}
% Consider a linear quadratic optimal control problem where system disturbances are mostly small but  occasionally large enough to cause input or state constraint violation, which we shall dub as safety constraints.
Consider a control problem where we wish to minimize an \textit{average} LQR cost, but also want that the closed loop meets certain safety guarantees against a set of rare yet possible \textit{worst-case} disturbances. Ideally, we would like to synthesize a controller that can guarantee the necessary safety constraints without too much loss in performance compared to the unconstrained LQR controller.

We will phrase this design goal as the following constrained LQR problem:
\begin{subequations}
\label{eq:const-lqr}
\begin{align}
\label{eq:cost-lqr}&\min_{\b{K}}\lim_{T \rightarrow \infty}\frac1T \sum_{t=1}^T \mathbb{E}_{w_t^i \sim p(w)}[\mathcal{J}(x_t,u_t) ] \\
&s.t.\,\,\,\,\,\,\,\,\,\,\,\, x_{t+1} = Ax_{t}+Bu_t + w_t\label{eq:lin-dyn}\\
 &\qquad  \,\,\,\,\,\,\,\,\,\,\,\,\,\,\,u_t = \b{K}(x_{t:0})\\
 & \qquad \forall \b{w}: \sup_k||w_k||_{\infty}\leq \eta_{max}:  \\
\label{eq:XUconstlqr}&\,\,\,\,\,\,\,\,\,\,\,\,\,\qquad  \sup_k ||x_k||_{\infty}\leq x_{max} \quad \sup_k ||u_k||_{\infty}\leq u_{max}  \nonumber
% \\
%\label{eq:Uconstlqr}&\,\,\,\,\,\,\,\,\,\,\,\,\, \qquad  \sup_k ||u_k||_{\infty}\leq u_{max} 
\end{align}
\end{subequations}
where $\mathcal{J}$ abbreviates the quadratic stage cost $\mathcal{J}(x,u) = x^TQx+uPu$ with $Q$,$P \succ 0$. Moreover, we will assume that the disturbance is stochastic but bounded and satisfies $\|w_k\|_{\infty} \leq \eta_{max}$ for all time $k$. Let the distribution of the disturbance be known and for ease of exposition, we will make the following additional assumption:
\begin{asp}
\label{assum:distribution}
Disturbance $w_t^i$ are i.i.d. drawn from the scalar centered distribution $p(w)$ and uncorrelated in time $t$ and coordinate $i$.
%$$ \E [w_t^i w_{t'}^j] = 0  \quad \forall i\not = j, t\not = t'$$
% In addition, we assume a bound on $w_k^i$, $\forall k,i$ such that $||w_k^i||\leq \eta_2$.
\end{asp}
More formally, we can use the system level framework introduced in \secref{sec:nlsls} to write the optimal control problem \eqref{eq:const-lqr} equivalently as an optimization over all characterizing CLMs $\CLM{x}$ and $\CLM{u}$ of the dynamics by recalling \thmref{thm:sufnec}:
\begin{subequations}
\label{eq:const-lqrclm}
\begin{align}
\label{eq:cost-lqrclm-cost2}&\min_{\CLM{x},\CLM{u}}\lim_{T \rightarrow \infty}\frac1T \sum_{t=1}^T \mathbb{E}[\mathcal{J}(\clm{x}{t}(w_{t:0}),\clm{u}{t}(w_{t:0})) ]
 \\
\label{eq:const-lqrclm-constclm2} &s.t. \,\,\, \,\,\,\,\,\,\,\, \clm{x}{t}(w_{t:0}) = \clm{x}{t}(0,0,w_{t-2:0}) + w_{t-1} \\
\nonumber&\clm{x}{t+1}(0,0,w_{t-1:0}) = A\clm{x}{t}(0,w_{t-1:0})+B\clm{u}{t}(0,w_{t-1:0})\\
 \label{eq:const-lqrclm-constx2} &\qquad \forall t, \|w_t\|_{\infty} \leq \eta_{max}:\quad \|\clm{x}{t}(w_{t:0})\|_{\infty} \leq x_{\mathrm{max}} \\
  \label{eq:const-lqrclm-constu2} &\qquad \forall t, \|w_t\|_{\infty} \leq \eta_{max}:\quad \|\clm{u}{t}(w_{t:0})\|_{\infty} \leq u_{\mathrm{max}} 
\end{align}
\end{subequations}
% \begin{subequations}
% \label{eq:const-lqrclm}
% \begin{align}
% \label{eq:cost-lqrclm-cost}&\min_{\b{K}}\lim_{T \rightarrow \infty}\frac1T \sum_{t=1}^T \mathbb{E}_{w_t^i \sim p(w)}[\mathcal{J}(\clm{x}{t}(w_{t:0}),\clm{u}{t}(w_{t:0})) ] \\
% \label{eq:const-lqrclm-constclm} &s.t.\,\,\, \CLM{x} = \CLMofFK{x}{Ax+Bu}{\b{K}},\quad \CLM{u} = \CLMofFK{u}{Ax+Bu}{\b{K}}\\
%  \label{eq:const-lqrclm-constx} &\qquad \forall t, \|w_t\|_{\infty} \leq \eta_{2}:\quad \|\clm{x}{t}(w_{t:0})\|_{\infty} \leq x_{\mathrm{max}} \\
%   \label{eq:const-lqrclm-constu} &\qquad \forall t, \|w_t\|_{\infty} \leq \eta_{2}:\quad \|\clm{u}{t}(w_{t:0})\|_{\infty} \leq u_{\mathrm{max}} 
% \end{align}
% \end{subequations}
% Furthermore,

As in the linear SLS case \cite{anderson2019system}, we do not need to have the controller $\b{K}$ be a decision variable, since we can always realize the optimal solution $\{\b{\Psi}^{(x)*},\b{\Psi}^{(u)*}\}$ to \eqref{eq:const-lqrclm} with a system level controller $\SL{\b{\Psi}^{(x)*}}{\b{\Psi}^{(u)*}}$.
% For the rest of the paper, we further assume weighting matrices $Q$ and $R$ to be identity to avoid overloading notation.
% Consider scenarios where the disturbances are mostly small but occasionally large enough to cause input or state constraint violation, which we shall dub as safety constraints. One naturally would wish to minimize the \textit{average} LQR cost while ensure safety constraints against the \textit{worst-case} albeit \textit{infrequent} disturbance. When disturbances are not adversarial and rarely achieve the worst-case norm, the controller synthesis procedure should exploit such knowledge. We capture this intuition by assuming disturbances are drawn from a centered distribution, $p(w)$ with bounded support. Without loss of generality, we make the assumption about disturbance below for simplicity of exposition. Note that the upcoming analysis can be carried out without it:
% \begin{asp}
% \label{assum:distribution}
% Disturbance $w_k^i$ are i.i.d. drawn from the scalar distribution $p(w)$ and uncorrelated in time and location, \textit{i.e.},
% $$ \E [w_t^i w_{t'}^j] = 0  \quad \forall i\not = j, t\not = t'$$
% In addition, we assume a bound on $w_k^i$, $\forall k,i$ such that $||w_k^i||\leq \eta_2$.
% \end{asp}

% Denote the LQR stage cost $\mathcal{J}_t(x_t,u_t) = x_t^TQx_t+u_tPu_t$, we aim to solve the following constrained LQR problem:
% \begin{subequations}
% \label{eq:const-lqr}
% \begin{align}
% \label{eq:cost-lqr}\min_{\b{K}} &\lim_{T \rightarrow \infty}\frac1T \sum_{t=1}^T \mathbb{E}_{w_t^i \sim p(w)}[\mathcal{J}_t(x_t,u_t) ] \\
% s.t.&\,\,\,\,\,\,\,\,\,\,\,\, x_{t+1} = Ax_{t}+Bu_t + w_t\label{eq:lin-dyn}\\
%  &\qquad  \,\,\,\,\,\,u_t = \b{K}(x_{t:0})\\
% & \forall w_k\text{ , } \forall k \in \mathbb{N}:  \left\|w_k \right\|_{\infty} \leq \eta_2 \text{ , }  \nonumber\\
% \label{eq:Xconstlqr}& \quad ||x_k||_{\infty} \leq x_{max} \quad \forall k\\
% \label{eq:Uconstlqr}& \quad  ||u_k ||_{\infty} \leq u_{max} \quad \forall k
% \end{align}
% \end{subequations}

% To avoid overloading notations, we also adopt the following assumption:
% \begin{asp}
% \label{assum:C+D}
% $Q = I$ and $P = I$.
% \end{asp}
% We aim to synthesize nonlinear  controller for a large scale linear systems with input and state constraints. The input constraints are assumed to be decentralized saturation-type constraints such that $\|u_t\|_{\infty}\leq u_{max}$ and the state constraints to be $\|x_t\|_{\infty}\leq x_{max}$\footnote{General polytopic input and state constraints can be similarly considered as in the sequel.}.



% Often the disturbances are mostly small, but occasionally large enough to cause safety violation. Therefore it is natural to have different control objectives depending on if we are facing small disturbances or large disturbances:
%  \begin{itemize}
% \item  (O1): If $w_k$ is small such that state constraint is guaranteed and input saturation does not happen, we want to prioritize performance with a \textit{performance-oriented} control strategy.
% \item (O2): If $w_k$ is large, we want to control in a \textit{safety-oriented} fashion by enforcing the input and state constraints. 
% \end{itemize}  


% For example, $p(w)$ could be multivariate truncated Gaussian distribution with estimated variance.
\subsection{Conservativeness of Linear Solutions}\label{sec:linneg}
We will first discuss properties of solutions to our original problem \eqref{eq:const-lqr}, if we restrict ourselves to only linear controllers $\b{K}$. As shown previously we can consider the equivalent problem formulation \eqref{eq:const-lqrclm}, where we restrict the CLMs $\{\CLM{x},\CLM{u}\}$ to be linear. This poses a convex problem and as shown in \cite{SLSChenAnderson2019}, it can be solved by searching over FIR CLMs $\{\CLM{x},\CLM{u}\}$ with large enough horizon $T$ and a realizing controller is $\SL{\CLM{x}}{\CLM{u}}$. Yet, the corresponding linear optimal CLMs $\{\CLM{x,lin*},\CLM{u,lin*}\}$ come with undesirable restrictions:

\begin{itemize}
    \item $\{\CLM{x,lin*},\CLM{u,lin*}\}$ impose stricter safety constraints than the required constraints \eqref{eq:const-lqrclm-constx2} and \eqref{eq:const-lqrclm-constu2}. 
    \item $\{\CLM{x,lin*},\CLM{u,lin*}\}$ do not depend on the disturbance distribution $p(w)$. 
\end{itemize}

To see the first point, we have the following result as a consequence of linearity:
\begin{lem}
For any linear $\{\CLM{x,lin},\CLM{u,lin}\}$, the constraint \eqref{eq:const-lqrclm-constx2},\eqref{eq:const-lqrclm-constu2} is equivalent to
\begin{subequations}
\label{eq:strict}
\begin{align}
\sup_t \|\clm{x,lin}{t}(w_{t:0})\|_{\infty} &\leq \sup_t \|w_t\|_{\infty} \frac{x_{max}}{\eta_{max}}\\
\sup_t \|\clm{u,lin}{t}(w_{t:0})\|_{\infty} &\leq \sup_t \|w_t\|_{\infty} \frac{u_{max}}{\eta_{max}}
\end{align}
\end{subequations}
\end{lem}
\begin{proof}
Clearly, \eqref{eq:strict} implies \eqref{eq:const-lqrclm-constx2},\eqref{eq:const-lqrclm-constu2}. The reverse implication follows by the assumed linearity of $\{\CLM{x,lin},\CLM{u,lin}\}$ and homogeneity of norms.
\end{proof}
To elaborate on the second point, notice that for linear CLMs $\CLM{x,lin},\CLM{u,lin}$ our objective function \eqref{eq:cost-lqrclm-cost2} can be expressed equivalently as 
\begin{align}\label{eq:H2simplify}
    \eqref{eq:cost-lqrclm-cost2} = \sigma^2\left\|\begin{array}{c}Q^{1/2} \CLM{x}\\ P^{1/2}\CLM{u} \end{array} \right\|^2_{\mathcal{H}_2},\quad \sigma^2:=\E_{w \sim p(w)}[w^2]
\end{align}
where $\sigma^2$ denotes the variance of the scalar distribution $p(w)$ and $\|.\|_{\mathcal{H}_2}$ denotes the $\mathcal{H}_2$ norm for linear operators. Since the objective function only gets scaled by a constant factor $\sigma^2$ for different distributions $p(w)$, this shows that for linear CLMs, the solutions $\{\CLM{x,lin},\CLM{u,lin}\}$ to \eqref{eq:const-lqrclm} are independent of the distribution $p(w)$. 

% To elaborate on the second point, we first note that the optimal solution to \eqref{eq:const-lqr} can be equivalently recovered by solving for the optimal linear CLM to \eqref{eq:lin-dyn}. Applying \assref{assum:distribution} and casting objective function \eqref{eq:cost-lqr} in terms of linear CLM of the form \eqref{eq:linear-maps} where $\b{x} = \b{R}\b{w}$ and ,$\b{u} = \b{M}\b{w}$ with $\b{R} = [R_1, R_2,\dots]$ and $\b{M} = [M_1, M_2,\dots]$ the linear operator, we have:
% \begin{align}
% \eqref{eq:cost-lqr}= 
% \E[(w_t^i)^2] \cdot \Trace  \left( \b{R}^T\b{R} +  \b{M}^T\b{M}  \right) 
% \end{align}

%In summary, a linear approach to problem \eqref{eq:const-lqr} not only has the drawback that the resulting closed loop will enforce safety constraints that are too conservative, but will completely ignore knowledge of the disturbance $p(w)$ during synthesis. In contrast, in many applications the disturbance can be assumed to be mostly small and only occasionally achieve worst-case size and it is conceivable that there should be a way to exploit this knowledge for control synthesis.


% We will see that especially when the variance of the disturbance is small, the optimal blended controller can offer a big improvement over linear optimal controllers.

%As we will see in the later sections, due to the former restrictions a linear controller will act to 
% Since solving the constrained LQR problem without expectation over $w$ is the same as solving one with given $p(w)$, the information about distribution is lost in the optimization over linear $\b{K}$ due to linearity.
% \begin{subequations}
% \label{eq:const-sls}
% \begin{align}
% \label{eq:costsls}\min_{\{\R1{k},\M1{k}\}_{k = 1:T}} &  \E[(w_t^i)^2] \cdot \Trace  \left( \begin{bmatrix} \R1{T:1} \\ \M1{T:1} \end{bmatrix} \begin{bmatrix} \R1{T:1} \\ \M1{T:1} \end{bmatrix}^T  \right)  \\
% s.t.&\,\,\,\,\,\,\,\,\, R_{k+1} = AR_{k} + BM_k \label{lin-sls-1}\\
% &\,\,\,\,\,\,\,\,\, R_{1} = I\label{lin-sls-2}\\
% &\,\,\,\,\,\,\,\,\, R_{T} = 0\label{lin-sls-3}\\
% & \forall w_k, k = 1,\dots,T,  \text{ with }  \left\|w_k \right\|_{\infty} \leq \eta: \nonumber\\
% \label{eq:Xconstsls}& \quad ||\sum_{k = 0}^{T-1} R_k w_{T-k}||_{\infty} \leq x_{max} \\
% \label{eq:Uconstsls}& \quad  ||\sum_{k = 0}^{T-1} M_k w_{T-k} ||_{\infty} \leq u_{max}
% \end{align}
% \end{subequations}
% To see the equivalence, note that \eqref{lin-sls-1}-\eqref{lin-sls-3} are the feasibility test for FIR linear CLM $\{\R1{k},\M1{k}\}_{k = 1:T}$. 


% We will refer to the above linear SLS constrained LQR problem as $\pro{\eta}$ since the solutions will have different properties depending on the value of $\eta$. On the one extreme, the centralized and distributed solution with $\eta=\eta_2$ was given in \cite{SLSChenAnderson2019} but we are optimizing for the worst-case performance. We call the solution to $\pro{\eta_2}$ the safe controller. On the other extreme, if we choose $\eta=\epsilon$ for small $\epsilon$, then  we will essentially obtain the optimal SLS controller as detailed in \cite{wang2019system} without the constraints \eqref{eq:Xconstsls} and \eqref{eq:Uconstsls} for (O1).

% Nevertheless, we would not like the apply either of the two. As will be demonstrated in \secref{sec:sim}, performance (as measured by the optimal LQR cost degradation) caused by conservatism can result in a big gap between unconstrained optimal controller performance and safe controller performance.
% The above discussion calls for a control strategy that offers flexibility depending on the size of disturbance. Ideally, the controller could take advantage of small disturbance and prioritize performance while being conservative when disturbance becomes larger information. 

\subsection{A NLSLS Take}
\label{sec:nlsls-take}
% Consider the general problem \eqref{eq:const-lqrclm2}
% Here we will show that the proposed nonlinear blend controller \eqref{eq:NL-map}

% the general problem \eqref{eq:const-lqrclm2} \eqref{eq:NL-map}
Consider the general problem \eqref{eq:const-lqrclm}, where now we search over CLMs $\{\CLM{x},\CLM{u}\}$ of the form presented in \eqref{eq:NL-map} with the choice of $\eta_2= \eta_{max}$, some $\eta_1<\eta_2$, and a finite memory horizon $T$. Recall that $\{\CLM{x},\CLM{u}\}$ is a blending of two linear CLMs and has the form \eqref{eq:NL-map}. Restricting ourselves to this form of CLMs, allows us to derive the following convex problem which is a relaxation of the general problem  \eqref{eq:const-lqrclm}:
% \begin{subequations}
% \label{eq:NL-map2}
% \begin{align}
%     \clm{x}{t}( w_{t:0}) = \sum^{\min\{T,t\}}_{k=1} &\R1{k} \p{1}{w_{t-k}} + \nonumber \\
%     & \R2{k}(\p2{w_{t-k}} - \p1{w_{t-k}}) \label{eq:NL-map-1}\\
%     \clm{u}{t}(w_{t:0}) = \sum^{\min\{T,t\}}_{k=1} &\M1{k} \p{1}{w_{t-k}} +\nonumber \\
%     & \M2{k}(\p2{w_{t-k}} - \p1{w_{t-k}}) \label{eq:NL-map-2}
% \end{align}
% \end{subequations}
% where $\{\R1{k}$, $\M1{k}\}_{k = 1:T}$ and $\{\R2{k}$, $\M2{k}\}_{k = 1:T}$ are the corresponding matrices of the linear CLMs $\{\CLM{x,1},\CLM{u,1}\}$ and  $\{\CLM{x,2}\CLM{u,2}\}$.
\begin{subequations}
\label{eq:S2}
\begin{align}
 \label{eq:cost-blend} \min_{\R{i}{}, \M{i}{}} & \left\|\begin{bmatrix} Q&0\\ 0 & P\end{bmatrix}^{1/2} \begin{bmatrix} \R1{} & \R2{} \\ \M1{}&\M2{}\end{bmatrix} \Sigma^{1/2}_w \right\|^{2}_{F}  \\
\label{eq:safety-1} 
s.t.\quad& \eta_1\|\R1{}\|_{\infty} + (\eta_2 - \eta_1)\|\R2{}\|_{\infty} \leq x_{max}\\
 &\eta_1\|\M1{}\|_{\infty} + (\eta_2 - \eta_1)\|\M2{}\|_{\infty} \leq u_{max} \label{eq:safety-2}\\
 & \R{i}{k+1} = A\R{i}{k} + B\M{i}k \label{lin-feas1}\\
 & \R{i}{1} = I,\quad \R{i}{T} = 0  \nonumber
\end{align}
\end{subequations}
where 
\begin{equation}
\label{eq:sigma} 
      \Sigma_w = \begin{bmatrix} \alpha_1 I & \alpha_2 I \\ \alpha_2 I &  \alpha_3 I  \end{bmatrix} \nonumber
    % \nonumber\\
    % \alpha_1 &= \E[\p1{w_t^i}^2]\nonumber \\
    % \alpha_2 &= \E[\p1{w_t^i} (\p2{w} -\p1{w_t^i})] \nonumber \\
    % \alpha_3 &= \E[(\p2{w_t^i} - \p1{w_t^i})^2] \nonumber\\
%       c_x &= ||[\R1T \R1{T-1} \R1{T-2} \dots \R11]||_{\infty}  \nonumber\\
%  c_u &= ||[\M1T \M1{T-1} \M1{T-2} \dots \M11]||_{\infty}   \nonumber
\end{equation}
with $\alpha_1 = \E[\p1{w}^2]$, $\alpha_2 = \E[\p1{w} (\p2{w} -\p1{w})]$, and $\alpha_3 = \E[(\p2{w} - \p1{w})^2]$, where $w \sim p(w)$. Moreover $\R{i}{}$ and $\M{i}{}$ are abbreviations for the row-wise concatenation of the matrices associated with the linear CLMs $\CLM{x,i}$, $\CLM{u,i}$, \textit{i.e}, $\R{i}{} = [\R{i}{T}, \R{i}{T-1}, \dots ,\R{i}{1}]$, $\M{i}{} = [\M{i}{T}, \M{i}{T-1}, \dots ,\M{i}{1}]$. Hereby, only constraints \eqref{eq:safety-1}, \eqref{eq:safety-2} are sufficient condition of the constraint \eqref{eq:const-lqrclm-constx2}, \eqref{eq:const-lqrclm-constu2} via norm multiplicativity. All other equations in the optimization are equivalent to the original optimization. Finally, solving the convex problem \eqref{eq:S2} gives us the sub-optimal nonlinear CLMs $\{\CLM{*x}, \CLM{*u}\}$ for the system dynamics \eqref{eq:lin-dyn}, which can be realized with the internally stabilizing system level controller $\SL{\CLM{*x}}{\CLM{*u}}$.
% Considering the following optimization over the linear CLM $\CLM{x,1}$,$\CLM{u,1}$ and $\CLM{x,2}$,$\CLM{u,2}$ for fixed $\eta_1 \in [0,\eta_2]$. Define row-wise concatenated matrices $\R{i} = [\R{i}{T}, \R{i}{T-1}, \dots ,\R{i}{1}]$, $\M{i} = [\M{i}{T}, \M{i}{T-1}, \dots ,\M{i}{1}]$
%Synthesis \eqref{eq:S2} jointly optimizes two linear CLM such that the nonlinear CLM \eqref{eq:NL-map2} still ensures the overall safety of the closed loop.
% The objective function \eqref{eq:cost-blend} is a \textit{equivalent} to the objective function of \eqref{eq:cost-lqrclm-cost2} by plugging \eqref{eq:NL-map2} into \eqref{eq:cost-lqr}. The safety constraint \eqref{eq:XUconstlqr} is relaxed through norm submultiplicativity to \eqref{eq:safety-1} and \eqref{eq:safety-2}. It is also straightforward to see that \eqref{eq:NL-map2} is an FIR CLM for dynamics \eqref{eq:lin-dyn} if and only if $\CLM{x,1}$,$\CLM{u,1}$,$\CLM{x,2}$,$\CLM{u,2}$ satisfy linear FIR CLM feasibility constraint \eqref{lin-feas1}-\eqref{lin-feas3}. 
%The nonlinear controller $\SL{\CLM{x}}{\CLM{u}}$ can then be constructed as a special case of \eqref{eq:SLeq} from the CLM synthesized in \eqref{eq:S2}:
% \begin{subequations}
% \label{eq:optimalblend}
% \begin{align}
%     \hat{w}_t &= x_t -\hat{x}_t\label{eq:global-1}\\
%     u_t &=  \clm{*u}{t}(0,\hat{w}_{t:t-T+1})\\
%     \hat{x}_{t} &=  \clm{*x}{t}(0,0,\hat{w}_{t-1:t-T+1})
% \end{align}
% \end{subequations}
% where $\{\CLM{*x}, \CLM{*u}\}$ denote the operators of the form \eqref{eq:NL-map}, with $\R{i}{}$, $\M{i}{}$ replaced by the solutions $\R{*i}{}$, $\M{*i}{}$ of the problem \eqref{eq:S2}.
% \begin{subequations}
% \begin{align}
% \label{eq:short-hand}
% \clm{*u}{t}(0,\hat{w}_{t:t-T+1})= \sum^{T-1}_{\tau = 0} &\M{*1}{\tau+1} \p1{\hat{w}_{t-\tau}} + \nonumber\\ &\M{*2}{\tau+1}(\p2{\hat{w}_{t-\tau}}-\p1{\hat{w}_{t-\tau}})\\
% \clm{*x}{t}(0,\hat{w}_{t:t-T+1}) = \sum^{T-1}_{\tau = 0} &\R{*1}{\tau+1}  \p1{\hat{w}_{t-\tau}} +\nonumber\\ 
% &\R{*2}{\tau+1}(\p2{\hat{w}_{t-\tau}}-\p1{\hat{w}_{t-\tau}})
% \end{align}\end{subequations}
% Note that we can freely choose $\eta_1$ as a hyperparameter. For the special case when $\eta_1$ is $0$, blending controller $\SL{\CLM{x}}{\CLM{u}}$ recovers linear \textit{safe} controller $\SL{\CLM{x,2}}{\CLM{u,2}}$ as the linear solution to \eqref{eq:const-lqr}. On the other hand, if $\eta_1$ fixed to be $(\eta_2-\epsilon)$, with $\epsilon$ arbitrarily small \footnote{This is to ensure \eqref{eq:safety-1} and \eqref{eq:safety-2} are well-defined.}, then constraints \eqref{eq:safety-1} and \eqref{eq:safety-2} could be arbitrarily relaxed, resulting in an arbitrary approximation to the performance controller $\SL{\CLM{x,1}}{\CLM{u,1}}$ as a solution to the unconstrained LQR problem. Therefore, $\eta_1$ serves as a tuning knob that balances the final blending controller to lie between pure performance-based strategy and the conservative safe strategy depending on whether estimated disturbance is small.
The next theorem states a main result of this paper: The synthesized controller $\SL{\CLM{*x}}{\CLM{*u}}$ from \eqref{eq:S2} outperforms any optimal linear controller for the constrained LQR problem.
\begin{thm}\label{thm:nlslsvssls}
For all $\eta_1 \in [0,\eta_2]$, the nonlinear system level controller $\SL{\CLM{*x}}{\CLM{*u}}$ achieves lower optimal LQR cost for \eqref{eq:const-lqr} than any linear solution to \eqref{eq:const-lqr}.
\end{thm}
\begin{proof}
First, recall that restricting $\b{K}$ to be linear in problem \eqref{eq:const-lqr} is equivalent to restricting $\CLM{x}$ and $\CLM{u}$ to be linear in the equivalent formulation \eqref{eq:const-lqrclm}. Furthermore, notice that under the restriction of linear $\{\CLM{x}, \CLM{u}\}$, problem \eqref{eq:const-lqrclm} is equivalent to \eqref{eq:S2} with the added constraint $\R1{} = \R2{}$, $\M1{}=\M2{}$, which proves that any solution $\{\CLM{*x}, \CLM{*u}\}$ of problem \eqref{eq:S2} achieve smaller cost than a linear solution $\{\CLM{x,lin*}, \CLM{u,lin*}\}$ of \eqref{eq:const-lqrclm}.
\end{proof}
%\begin{coro}\label{thm:n-nlslsvssls}
%The N-blend nonlinear system level controller $\SL{\CLM{x}}{\CLM{u}}$ of the form \eqref{eq:n-blend} constructed from the solution of \eqref{eq:S2} with \eqref{eq:safety-1} and \eqref{eq:safety-2} replaced with the following:
%\begin{subequations}
%\begin{align}
%&\sum_{i = 1}^N (\eta_i - \eta_{i-1})\|R^{(i)}\|_{\infty} \leq x_{max}\\
%&\sum_{i = 1}^N (\eta_i - \eta_{i-1})\|M^{(i)}\|_{\infty} \leq u_{max} 
% \end{align}
%\end{subequations}
%with  $\eta_{max} = \eta_N \geq\eta_{N-1} \geq \dots \geq \eta_0 =  0$
%achieves lower optimal LQR cost for \eqref{eq:const-lqr} than any linear solution to \eqref{eq:const-lqr}.
%\end{coro}
%\begin{proof}
%The same reasoning as \thmref{thm:nlslsvssls} applies.
%\end{proof}
\begin{coro}\label{thm:n-nlslsvssls}
	The N-blend nonlinear system level controller $\SL{\CLM{x}}{\CLM{u}}$ of the form \eqref{eq:n-blend} constructed from the solution of \eqref{eq:S2} for $N$ linear CLMs
	with  $\eta_{max} = \eta_N \geq\eta_{N-1} \geq \dots \geq \eta_0 =  0$
	achieves lower optimal LQR cost for \eqref{eq:const-lqr} than any linear solution to \eqref{eq:const-lqr}.
\end{coro}
\begin{proof}
	The same reasoning as the proof of \thmref{thm:nlslsvssls} applies.
\end{proof}


\subsection{Distributed Controller for Constrained LQR}
\label{sec:ls-lqr}
Thanks to the particular form of \eqref{eq:n-blend}, when the projection is chosen to be the saturation projection \defref{def:sat}, structural constraints of controller such as sparsity and delay constraints can be added in a convex way to the synthesis procedure described in \secref{sec:nlsls-take}. This is because imposing structural constraints on the nonlinear controller \eqref{eq:n-blend} is equivalent to imposing them on the linear CLM components of \eqref{eq:n-blend}. Detailed in \cite{anderson2019system}, localization of disturbance, communication and actuation delay, as well as sparsity pattern are all convex constraints in terms of linear CLMs in the linear System Level Synthesis framework. Specifically, all mentioned constraints could be cast as a convex subspace $\mathcal{S}_x$ and $\mathcal{S}_u$ for linear CLMs $\CLM{x,i}$,$\CLM{u,i}$,$i \in \set{N}$ in $\SL{\TU}{\TX}$. Therefore, the nonlinear controller synthesis in \secref{sec:nlsls-take} naturally inherits all capabilities of the linear system level controllers in terms of distributed controller syntehsis. 







==> [ACC2020] Saturation_Arxiv_ver/nlsls_v1.tex <==
 This section will focus on introducing the notion of closed loop maps as causal operators w.r.t. a general nonlinear causal system. Moreover, we summarize necessary and sufficient conditions for operators to be closed loop maps and how they can be realized by a dynamic controller\cite{NLSLSHODoyle2019}.

\subsection{Closed Loop Maps of Nonlinear Systems}
Consider a general discrete-time nonlinear system with additive noise
\begin{align} \label{eq:sys}
x_{t+1} = f(x_{t},u_{t}) +w_t
\end{align}
where $x_t\in \mathbb{R}^n$, $u_t\in \mathbb{R}^p$, $w_t\in \mathbb{R}^n$ and $f:\RR^{n \times \N} \times \RR^{p \times \N} \rightarrow \RR^{n \times \N}$ is a causal operator with zero initial condition. Assume that $w_t$ can not be measured and that $u_t$ is generated by some $\b{K}:\RR^{n\times \N} \rightarrow \RR^{p \times \N}$, i.e. $\b{u} = \b{K}(\b{x})$:
\begin{align}\label{eq:u}
u_t = K_t\left(x_{t:0} \right)
\end{align}



% Furthermore let's make the following smoothness assumption:
%\begin{asp}\label{asp:lip}
%$f(x,u)$ is Lipshitz w.r.t $x$ and $u$ with the step $L$.
%\end{asp}
For a fixed disturbance sequence $\b{w}$, the dynamics \eqref{eq:sys} produces unique closed loop trajectories for state $\b{x}$ and input $\b{u}$. Therefore, given a fixed $\b{K}$, the dynamics induce a causal map from $\b{w}$ to $\b{x}$, $\b{u}$ and we will call the corresponding operators disturbance-to-state and disturbance-to-input \textit{closed loop maps}, respectively:
\begin{defn}[Closed Loop Maps]\label{def:clm}
We will call the operators $\b{\Phi}^{\b{w} \rightarrow \b{x}}_{[f,\b{K}]}:\RR^{n \times \N} \rightarrow \RR^{p \times \N}$ and $\b{\Phi}^{\b{w} \rightarrow \b{u}}_{[f,\b{K}]}:\RR^{n \times \N} \rightarrow \RR^{p \times \N}$ 
the disturbance-to-state and disturbance-to-input closed-loop maps(CLMs) of system $f$ w.r.t. controller $\b{K}$ if they map disturbance sequences $\b{w}$ to the corresponding state and input sequences $\b{x}$, $\b{u}$ of the system \eqref{eq:sys}, \textit{i.e.},
\begin{align}
&& x_{t+1} = f(x_{t},K_{t}(x_{t:0})) +w_t \\
&\Leftrightarrow &   \b{x} = \CLMofK{x}{\b{K}} (\b{w}), \quad \b{K}(\b{x}) = \CLMofK{u}{\b{K}}(\b{w})
\end{align}
we say the pair of operators $\{\CLM{x}$, $\CLM{u}\}$ is CLM of system \eqref{eq:sys}, if there exists a \textit{realizing} controller $\b{K}'$ such that
\begin{align}
&\CLM{x}=\CLMofK{x}{\b{K}'} &\CLM{u}=\CLMofK{u}{\b{K}'}
\end{align}
\end{defn}
The following theorem characterizes the space of CLMs for a given system $f$:
\begin{thm}\label{thm:sufnec}
$\CLM{x}$ and $\CLM{u}$ are CLMs of \eqref{eq:sys} if and only if they satisfy the following functional equations for all time $t$.
\begin{align}
\label{eq:feasnl}
\clm{x}{t}(w_{t:0}) &= \clm{x}{t}(0,0,w_{t-2:0}) + w_{t-1}\\
\label{eq:opfunceq_red}\clm{x}{t+1}(0,0,w_{t-1:0}) &= f(\clm{x}{t:0}(0,w_{t-1:0}),\clm{u}{t:0}(0,w_{t-1:0})) \nonumber
\end{align}
\end{thm}

%%%
\subsection{System Level Controllers}
We will call the realizing controllers of CLM pair $\{\CLM{x},\CLM{u}\}$ the \textit{System Level} (SL)-controllers
\begin{defn}[SL Controller]\label{def:SL}
Given causal operators $\TX:\RR^{n \times \N} \rightarrow \RR^{n \times \N}$, $\TU:\RR^{n \times \N}\rightarrow \RR^{p \times \N}$ define the system level(SL) controller as the operator $\b{K}(\b{x}): \RR^{n \times \N} \rightarrow \RR^{p \times \N}$ with realization
%\begin{align}
%u_t = K_t(x_{t:0}) = \Tu{t}(0,\hat{w}_{t:1})
%\end{align}
%where $\hat{w}_t$ is computed through the recursion
%\begin{subequations}
%\label{eq:SLeq}
%\begin{align}
%\hat{w}_0 &= x_0\\
%\hat{w}_1 &= x_1-\Tx{1}(0,0)\\
%&\dots \nonumber\\
%\hat{w}_t &= x_t-\Tx{t}(0,0,\hat{w}_{t-1:1})
%\end{align}
%\end{subequations}
\begin{subequations}
	\label{eq:SLeq}
	\begin{align}
	u_t = K_t(x_{t:0}) &= \Tu{t}(0,\hat{w}_{t:1})\\
	\hat{w}_0 &= x_0\\
	\hat{w}_t &= x_t-\Tx{t}(0,0,\hat{w}_{t-1:1})
	\end{align}
\end{subequations}
We will write $\b{K}=\SL{\TX}{\TU}$ to underscore that an operator $\b{K}$ is the system level (SL) controller of the CLMs $\{\TX$, $\TU\}$ and will refer to $\hat{w}_t$ as the internal state of $\b{K}$.
\end{defn}

% Given any system-level controller $\b{K}=\SL{\TX}{\TU}$, define $\b{x}'$, $\b{u}'$ as the input and output of the operator, \textit{i.e.}, $\b{u}' = \b{K}(\b{x}')$. Then the SL controller preserves the following important relation between $\b{u}'$, $\b{x}'$ and it's internal state $\hat{\b{w}}$:
% \begin{subequations}
% \begin{align}\label{eq:invSL}
%     x'_t &= \Tx{t}\left(0,0,\hat{w}_{t-1:1}\right)+\hat{w}_{t}\\
%     u'_t &= \Tu{t}\left(0,\hat{w}_{t:1}\right)
% \end{align}
% \end{subequations}

% Consider the closed loop of the nonlinear system \eqref{eq:sys} with the SL-controller $u_t = K_t(x_{t:0}+v_{t:0})+d_t$ subject to bounded perturbations $\b{v}$ and $\b{d}$ in state and input. Using the above relation, the dynamics of the closed loop can be written as:
% \begin{subequations}
% \label{eq:cleq}\begin{align}
%   \label{eq:clint} \hat{w}_{t+1} &= \Delta_t(\hat{w}_{t:1},v_t,d_t) + w_t\\
%     \label{eq:clx}     x_t &= \Tx{t}\left(0,0,\hat{w}_{t-1:1}\right)+\hat{w}_{t}-v_t\\
%     \label{eq:clu}u_t &= \Tu{t}\left(0,\hat{w}_{t:1}\right)+d_t
% \end{align}
% \end{subequations}
% where $\b{\Delta}$ stands for the operator:
% \begin{align}
%     \notag \Delta_t(&\hat{w}_{t:1},v_t,d_t):= f(\Tx{t:0}(0,\hat{w}_{t:1})-v_t, \\
%     \label{eq:Delta} &\Tu{t:0}(0,\hat{w}_{t:1})+d_t) - \Tx{t+1}\left(0,0,\hat{w}_{t:1}\right)
% \end{align}


% \begin{thm}[Realizing Controller of CLMs\cite{NLSLSHODoyle2019}]\label{thm:real}
% \phantom{as} Consider the dynamics \eqref{eq:cleq} of the system \eqref{eq:sys} in closed loop with an SL-controller $\b{K} = \SL{\CLM{x}}{\CLM{u}}$. Then, if $\CLM{x}$ and $\CLM{u}$ are CLMs of \eqref{eq:sys}, then $\CLMofK{x}{\b{K}} = \CLM{x}$ and $\CLMofK{u}{\b{K}} = \CLM{u}$.
%  \end{thm}
 \begin{thm}[Stability of Closed Loop\cite{NLSLSHODoyle2019}]\label{thm:stability}
If $f$ is uniformly continuous and the operators $\CLM{x},\CLM{u}$  are $\ell_p$-stable CLMs of \eqref{eq:sys} (or $\ell_p$ finite gain-stable), then the closed loop dynamics are $\ell_p$-stable (or finite gain $\ell_p$-stable) w.r.t to the bounded perturbations $\b{w}$, $\b{d}$ and $\b{v}$. 
% Moreover, if $\CLM{x},\CLM{u}$ are \textit{not} CLMs of the system \eqref{eq:sys}, then the previous stability guarantee still holds true if and only if the internal dynamics \label{eq:clint} are $\ell_p$-stable/finite gain $\ell_p$-stable. 
\end{thm}
%
%A particular subclass of stable operators that we will consider in this work are operators of finite memory, which are defined as follows:
%\begin{defn}[CLM with Finite Memory]\label{def:FM}
%CLM $\{\CLM{x},\CLM{u}\}$ are said to have finite memory of horizon $T$ if
%\begin{equation}
%    \clm{x}{t+1}(0,w_{t:0}) =
%    \begin{cases}
%    \clm{x}{t+1}(0,w_{t:0}) & \forall t < T \\
%        \clm{x}{t+1}(0,w_{t:t+1-T},0,\dots,0) & \forall t \geq T
%    \end{cases}
%\end{equation}
%
%\end{defn}
\subsection{Relation to Linear System Level Approach}
If we restrict the previous analysis to linear time-invariant (LTI) systems and controllers, we recover the results of \cite{anderson2019system} for the state-feedback case.
If $x_{t+1} = Ax_t + Bu_t + w_t$ and $\b{K}$ is a LTI operator, then the corresponding linear closed loop maps are LTI as well.
%With the abbreviation $\CLM{x} = \CLMofK{x}{\b{K}}$, $\CLM{u} = \CLMofK{x}{\b{K}}$, the CLM takes the realization
In this case, the CLMs take the realization
\begin{subequations}
\label{eq:linear-maps}
\begin{align}
    \clm{x}{t}(0,w_{t-1:0}) & = \sum^{t}_{k=1}R_k w_{t-k}\\
    \clm{x}{u}(0,w_{t-1:0}) & = \sum^{t}_{k=1}M_k w_{t-k}
\end{align}
\end{subequations}
where $R_k \in \RR^{n \times n}$, $M_k \in \RR^{p \times n}$ are called associated matrices of $\CLM{x}$ and $\CLM{u}$. Moreover, the corresponding CLM feasibility condition reduces to the affine constraint on the matrices $R_k$, $M_k$ which coincides with the linear System Level Synthesis(SLS) feasibility conditions derived in \cite{anderson2019system}. Let $\CLM{x}$ and $\CLM{u}$ be further constrained to have Finite Impulse Response (FIR) of horizon $T$, then parameterization of the CLMs in \eqref{eq:feasnl}  reduces to:
\begin{subequations}
\label{eq:lin-feaibility}
\begin{align}
    &R_{1} = I \\
    &R_{k+1} = A R_k + B M_k \\
    &A R_{T-1} + B M_{T-1} = 0
\end{align}
\end{subequations}
 Similarly, a strictly causal system level controller $\b{K} = \SL{\CLM{x}}{\CLM{u}}$ in \eqref{eq:SLeq} with LTI operators $\CLM{x}$, $\CLM{u}$ satisfying the above becomes 
\begin{align}
\hat{w}_t &= x_t - \sum^{\min\{t,T-1\}}_{k=1}R_{k+1}\hat{w}_{t-k}\\
\label{eq:nl-controller-2} u_t &=   \sum^{\min\{t,T-1\}}_{k=0}M_{k+1}\hat{w}_{t-k}
\end{align}
which describes the standard SLS controller in \cite{anderson2019system}. Since the CLMs are chosen to be FIR, internal stability of the closed-loop system is immediate.

% since by definition of CLMs, we have the following closed-loop behaviour:
%\begin{align}
%\label{eq:lin-controller}
%&x_{t} = \sum^{\min\{t,T\}}_{k=1}R_{k}w_{t-k},
%&u_{t} = \sum^{\min\{t,T\}}_{k=1}M_{k}w_{t-k}
%\end{align} 
%Recall from \cite{slsacc}, that linear CLMs $\CLM{x}$, $\CLM{u}$ are called finite impulse response(FIR) CLM of horizon $T$, if $R_T$, $M_T$ satisfy $$. The corresponding closed loop is then trivially stable since the closed loop has a finite impulse response and enforces the following CLM between the disturbance $\b{w}$ and $\b{x}$, $\b{u}$: 



==> [ACC2020] Saturation_Arxiv_ver/prelim_v1.tex <==
%We will use the following abbreviation whenever it will be cumbersome to write expressions with functions of many arguments: Define $f(x_{i:j})$ to be $f(x_{i},x_{i+1},\dots, x_{j})$ for ($i <j$) and $f(x_{i},x_{i-1},\dots, x_{j})$ for ($i >j$), respectively.  Unless otherwise specified, $||\cdot||$ denotes the infinity norm for vectors and induced infinity norm for matrices. 

 We will define  $\mathbb{R}^{n \times \mathbb{N}}$ to be spaces of sequences of vectors in $\RR^n$. A causal operator will be denoted in bold capital letters $\b{T}$ and will represent maps of the form $\RR^{n \times \N} \rightarrow \RR^{k \times \N}$.The corresponding functions that map $x_{t:0}$ to $(\b{T}(\b{x}))_t$ are denoted as $T_t:\RR^{n \times (t+1)} \rightarrow \RR^k $ and the realization of a causal operator is $\b{T}(\b{x})=(T_0(x_0), T_1(x_1,x_0),T_2(x_2,x_1,x_0), \dots)$.
% Denote column-wise concatenation through $\left[A;B \right] := \left[A^T,B^T\right]^T$.
 Sequences of vectors $(x_t)^{\infty}_{t=0}$ will be denoted by small bold letters $\b{x}$ unless otherwise specified and $\b{x}_t$ is the vector $x_t$ at $t$th time step in the sequence with $x^j_t$ denotes the $j$th element of vector $x_t$. We will use the notation $x_{i:j}$ to refer to the truncation of the sequence $[x_{i},x_{i+1},\dots, x_{j}]$. 
%  The transpose of truncated sequence of vectors is $x_{1:k}^T := [x_1^T,x_2^T,\dots, x_k^T]^T$.  
 Furthermore, we will adopt $\|.\|_{p}$ to refer to the $\ell _p$ norm and induced norm on vectors and matrices. The set of positive integers ranging from 1 to $N$ will be denoted as $\set{N}$.
% \begin{align}
% \ell^{n}_{p} &:= \left\{\b{x} \in \mathbb{R}^{n \times \mathbb{N}} \left| \Nxy{\b{s}}{p} < \infty, \quad s_k := \Nxy{x_k}{} \right. \right\} \\
% \Nxy{\b{x}}{p} & := \Nxy{(\Nxy{x_0}{},\Nxy{x_1}{},\dots)}{p}
% \end{align}
% In particular, $\ell^{n}_{\infty}$ denotes the space of all bounded sequences in the normed vector space $(\Nxy{.}{},\RR^n)$. 
%\subsection{Causal Operators}
% Operators will be denoted in bold capital letters $\b{T}$ and will represent maps of the form $\RR^{n \times \N} \rightarrow \RR^{k \times \N}$. An operator will be called causal if $(\b{T}(\b{x}))_t$ depends only on $x_{t:0}$. The corresponding functions that map $x_{t:0}$ to $(\b{T}(\b{x}))_t$ are denoted as $T_t:\RR^{n \times (t+1)} \rightarrow \RR^k $ and the realization of a causal operator is $\b{T}(\b{x})=(T_0(x_0), T_1(x_1,x_0),T_2(x_2,x_1,x_0), \dots)$.
% 
% \begin{defn}[ Stable Causal Operators]
%A causal operator $\b{T}:\RR^{n \times \N} \rightarrow \RR^{k \times \N}$ is defined to be $\ell_p$-stable if $\Nxy{\b{x}}{p} < \infty $ implies $\Nxy{\b{T}(\b{x})}{p} < \infty$ and \textit{finite gain} $\ell_p$-stable with gain $\gamma \geq 0$ if there exist $\beta \geq 0$  such that $\Nxy{\b{T}(\b{x})}{p} \leq  \gamma\Nxy{\b{x}}{p} + \beta $ for all $\b{x} \in \ell^n_p$.
%\end{defn}

% \begin{defn}[Causal Operator]\label{def:caus}
%  An operator $\b{T}:\RR^{n \times \N} \rightarrow \RR^{k \times \N}$ is \textit{causal}, if there exist functions $T_t:\RR^{n \times (t+1)} \rightarrow \RR^k$ such that $(\b{T}(\b{x}))_t = T_t(x_{t:0})$ for all $t$ and sequences $\b{x} \in \RR^{n \times \N}$. If in addition $T_t(x_{t:0}) = T_t(0,x_{t-1:0}) $ holds $\b{T}$ is called \textit{strictly causal}. Furthermore, let $T_{i:j}: \RR^{n \times (\max\{i,j\}+1)} \rightarrow \RR^{k \times (|j-i|+1)}$ be the truncation map defined as:
% \begin{align}
% T_{i:j}(x_{j:0}) &:= (\b{T}(\b{x}))_{i:j} \quad \text{for }j\geq i \\
% T_{i:j}(x_{i:0}) &:= (\b{T}(\b{x}))_{i:j} \quad \text{for }j<i.
% \end{align}
% \end{defn} 

%New Stuff
%%%%

==> [ACC2020] Saturation_Arxiv_ver/scalar_v1.tex <==
In this section, we will show that the simple projection nonlinearity in \eqref{eq:NL-map} gives the proposed nonlinear blending controller $\SL{\CLM{x}}{\CLM{u}}$  discussed in \secref{sec:blend} a natural anti-windup property. 
%In particular, it will be illustrated that $\SL{\CLM{x}}{\CLM{u}}$   recovers simple anti-windup schemes for integrator windup problem under input saturation. 
We choose a scalar case to start the analysis for ease of exposition.

Consider the following \textit{linear} controller design problem:
\begin{subequations}
\label{eq:scalar}
\begin{align}
\label{eq:costsls}\min_{\b{K}} &  \lim_{T \rightarrow \infty}\frac1T\sum_{k = 0}^{T} x^2 \\
s.t.\,\,\,\,\,\,\,\,\,  x_{t+1} &= x_{t} + u_t + w_t, \quad x_0 = 0\\
 u_t &= \b{K}(x_{t:0})\\
 \b{w} = \b{1}: \,\,\, x_t &= 0 \quad \forall t \geq 2   \label{eq:rpa}
\end{align}
\end{subequations}
The performance objective \eqref{eq:rpa} states that the system should return to origin within two time steps after a step disturbance hits. Such objective could only be fulfilled when the controller has an internal integrator where step disturbance can be perfectly rejected.

One can check that the optimal \textit{integral} SL-controller for \eqref{eq:scalar} is 
\begin{subequations}
\label{eq:rpa-controller}
\begin{align}
    \hat{w}_{t+1} &= \hat{w}_t +x_t\\
    u_t &= -x_t - \hat{w}_t
\end{align}
\end{subequations}
Because integral action is required to perfectly reject step input, input saturation could cause severe windup behaviour leading to instability. As shown in \figref{fig:scalar}, bounded sequence of disturbance between $-1$ and $1$ causes severe windup effects for integrator controller \eqref{eq:rpa-controller} under saturation: $\text{sat}(u_t) = \text{sign}(u_t)\min\{|u_t|,1\}$. 
The simplest strategy one could adopt in this case is to switch to a controller synthesized from \eqref{eq:scalar} without performance requirement \eqref{eq:rpa} in the face of saturation to ensure closed loop stability. Inspection of \eqref{eq:scalar} verifies the optimal \textit{non-integral} SL-controller is simply a deadbeat controller 
\begin{equation}
\label{eq:nonrpa-controller}
    u_t = -x_t
\end{equation}
% The simplest strategy one could adopt in this case is to "turn off" the integrator part of the controller, \textit{i.e.}, switching to $G_{aw}(z) = -2$ in the face of saturation to ensure closed loop stability. 
However, the non-integral controller does not satisfy the performance objective of step input rejection. Therefore, one naturally seeks a "middle ground" between \eqref{eq:rpa-controller} and \eqref{eq:nonrpa-controller} where under small signals, integral actions are taken to meet performance objective while guaranteeing stability under large signals.
\begin{figure}[h]
 \centering
 \includegraphics{scalar.pdf}
 \caption{Saturating response to large worst-case disturbance for the integral controller (dotted-red), anti-windup controller (blue), and naive blending controller (green): Integral controller becomes unstable in the face of input saturation. The response of simple anti-windup schemes that simply turn off the integral portion of the controller is recovered by the proposed naive blending controller.}
 \label{fig:scalar}
% \end{figure}

% \begin{figure}[h]
%  \centering
 \vspace{0.00cm}
 \includegraphics{scalar-db-vs-blend.pdf}
 \caption{Response of Simple Linear Anti-windup Controller (blue) VS. Proposed Blending (green) for small step Input: The simple linear anti-windup controller used globally ensures stability under saturation at the cost of forfeiting the step response performance objective. The naive blending controller recovers this performance objective in the case of small steps while still ensure stability under saturation.}
 \label{fig:db-vs-blend}
\end{figure}
Consider now the blending nonlinear controller $\SL{\CLM{x}}{\CLM{u}}$ from \eqref{eq:NL-map}. A naive scheme is simply blending the \textit{integral} and \textit{non-integral} controller with a small $\eta_1$ value. Denote the transformed controller internal state $\tilde{w}_t = \p{1}{\hat{w}_t}$, the resulting blending nonlinear SL-controller is:
\begin{subequations}
\label{eq:scala-blend}
\begin{align}
    \tilde{w}_{t+1} &= \p{1}{\tilde{w}_t + x_t}\\
    u_t &= -x_t-\tilde{w}_t
\end{align}
\end{subequations}
It is now clear that the projection nonlinearity in \eqref{eq:NL-map} offers a natural anti-windup property since the essence of traditional anti-windup schemes \cite{kothare1994unified} is to stop the integrator from accumulating errors. As demonstrated in \figref{fig:scalar} and \figref{fig:db-vs-blend}, the blending controller achieves similar stable behaviour as the non-integrator controller under controller saturation but recovers performance in the small-signal regime. 

For this scalar example, the projection nonlinearity of \eqref{eq:NL-map} automatically allow the naive blending scheme to have anti-windup property while preserving performance under small disturbance. Despite the simplicity of the projection nonlinearity in \eqref{eq:NL-map}, we will see in the next section that the anti-windup property for the naive blending scheme extends to the large-scale case.

==> [ACC2020] Saturation_Arxiv_ver/simulation_v1.tex <==
\subsection{Constrained LQR}
To corroborate the results presented in the previous sections, we demonstrate the performance of a four-zone nonlinear blending controller with radial projection compared against the optimal linear controller for the constrained LQR problem of an open-loop unstable system: 
\begin{align}
    x_{k+1} &= \begin{bmatrix}1&1&0\\1&2&1\\0&1&1 \end{bmatrix}x_k + \begin{bmatrix}0\\0\\1 \end{bmatrix}u_k +w_k
\end{align}
with $u_{max} = 40$, $x_{max} = 15$, $\eta_{max} = 1$, $Q = I_3$, $P = 10$. The disturbances $w_k$ are chosen to be a truncated i.i.d. gaussian random variables with variance $\sigma^2$. \figref{fig:performance} shows the optimal cost improvement of the presented nonlinear approach over the optimal linear controller for different choices of variance $\sigma^2$. \figref{fig:performance} showcases that the proposed controller can exploit the knowledge of the disturbance distribution to achieve performance improvement over the linear optimal linear controller: For small $\sigma$ the proposed controller gains more than 30\% cost reduction over safe controller. On the other hand, with increasing $\sigma$, large disturbances in the system become more likely, and therefore the opportunity to improve upon the linear optimal controller is reduced.
\begin{figure}[h]
 \centering
 \includegraphics[scale = 0.75]{figure/performance_1.pdf}
 \caption{Performance improvement of optimal nonlinear controller $\SL{\CLM{*x}}{\CLM{*u}}$ over optimal linear controller $\SL{\CLM{x,lin*}}{\CLM{u,lin*}}$ for different variances $\sigma^2$ of the non-truncated disturbance. The nonlinear blending controller synthesizes over 4 linear controllers w.r.t. to the projection parameters $\eta_1= 0.05, \eta_2 = 0.1, \eta_3 = 0.2, \eta_4 = \eta_{max} = 1 $}
 \label{fig:performance}
\end{figure}

\subsection{Distributed Anti-Windup Controller}
Consider a bi-directional chain system with $i$th node's dynamics being
\begin{equation}
\label{eqn:sim}
    x^i_{t+1} = (1- 0.4\lvert \mathcal{N}(i) \rvert  ) x^i_t + 0.4 \sum_{j \in \mathcal{N}_i} x^j_t + \sat(u^i_t,u_{max}) + w_t^i \nonumber
\end{equation}
where $\mathcal{N}(i)$ denotes the set of vertices that has an edge connected to $i$th vertex and $w_t^i$ is the $i$th coordinate of disturbance vector at time $t$. In particular, $\|\b{w}\|_{\infty}\leq 1$ and $x_0 = 0$.  One can check that the overall chain system is open-loop marginally stable.

We illustrate the anti-windup property of the nonlinear controller \eqref{eq:n-blend} in the decentralized setting with additional sparsity, locality, and delay constraints. First, a nominal integral controller for this system is designed and dubbed as the \textit{Integral Controller}. Due to its integral structure, the \textit{Integral Controller} for the unconstrained closed loop guarantees convergence of the state to the origin under persistent disturbance, \textit{i.e}, step rejection. In comparison, a second linear controller synthesized from standard constrained LQR problem that guarantees stability for all admissible $\b{w}$ under saturation is generated. We refer to this linear controller as the \textit{Non-integral Controller} since the states only stay bounded under persistent admissable disturbance.  

 The nonlinear controller with saturation projection here is chosen to be a two-zone blending controller consisted of CLMs of the form \eqref{eq:NL-map}. The simulation shows the anti-windup property as well as preservation of step rejection in both large- and small-disturbance schemes of the proposed method. \figref{fig:ls-worst} shows that the blending controller stabilizes the system while integral controller becomes unstable under worst-case bounded disturbance. On the other hand, the proposed blending controller preserves performance of step rejection while the linear Non-integral Controllers forfeits the performance objective in order to preserve stability in the saturated closed loop. In this chain example, we allow 1 time step communication delay between nodes and actuation delay with 50\% control authority. The localization pattern imposed on the system response allows $\SL{\CLM{x}}{ \CLM{u}}$ to be implemented in local patches, therefore making the controller distributed.
% \begin{equation}
% \label{eqn:sim}
%     x^i_{t+1} = \rho (1-\lvert \mathcal{N}(i) \rvert \alpha ) x^i_t + \rho \alpha \sum_{j \in \mathcal{N}_i} x^j_t + u^i_t
% \end{equation}




\begin{figure*}
\centering
%   \subfigure[Integral Controller under Worst-case Disturbance/under Staggered Step Disturbance]{ \includegraphics[scale = 0.5, trim = 5cm 7.8cm 6cm 7.8cm, clip]{worst-rpa.pdf}}
 \subfigure[Integral Controller]{ \includegraphics{figure/worst-rpa.pdf}}
%  \caption{Response of Integral Controller}
  \subfigure[Non-integral Controller]{ \includegraphics{figure/worst-nonrpa.pdf}\label{fig:ls-act}}
    \subfigure[Nonlinear Blending Controller ]{ \includegraphics{figure/worst-blend.pdf}\label{fig:ls-act}}
     % \subfigure[Integral Controller ]{ \includegraphics[scale = 0.48, trim = 5cm 8.5cm 6cm 8.5cm, clip]{step-rpa.pdf}}
     \subfigure[Integral Controller ]{ \includegraphics{figure/step-rpa.pdf}}   
%  \caption{Response of Integral Controller}
  \subfigure[Non-integral Controller ]{ \includegraphics{figure/step-nonrpa.pdf}\label{fig:ls-act}}
    \subfigure[Nonlinear Blending Controller ]{ \includegraphics{figure/step-blend.pdf}\label{fig:ls-act}}
   \caption{\textit{\textbf{Worst-case (top row) and Staggered Step Input (bottom row) Response} under Saturation for a marginally stable 20-node Chain System with Sparse Actuation}: \textit{Top Row}: Worst-case disturbance propagates through space-time for the saturated chain system. The nonlinear controller possesses the anti-windup property of the non-integral controller. In addition to  anti-windup, the proposed controller is localized and accommodates sparse actuation, communication delay, and controller sparsity constraints. Here every other node has a control input (50\% actuation) with 1 time step actuation delay and 1 time step communication delay between nodes, while enforcing a controller sparsity that conforms to the communication pattern of dynamics matrix $A$. \textit{Bottom Row}: Response to small step disturbances at node 8,10,12 entering at time 2,6,10, respectively.The blending controller not only stabilizes under saturation but also recovers the performance objective of rejecting small step disturbances. 
}
   \label{fig:ls-worst}
\end{figure*} 

%Worst-case (top row) and Staggered Step Input (bottom row) Response} under Saturation for a marginally stable 20-node Chain System with Sparse Actuation}: \textit{Top Row}: The heatmaps show how a worst-case disturbance is propagated through space-time for the saturated chain system. The integral controller becomes unstable due to saturation and the nonlinear controller possesses the anti-windup property of the non-integral controller.
%In addition to  anti-windup, the proposed controller is localized and accommodates sparse actuation, communication delay, and controller sparsity constraints. Here every other node has a control input (50\% actuation) with 1 time step actuation delay and 1 time step communication delay between nodes, while enforcing a controller sparsity that conforms to the communication pattern of dynamics matrix $A$. \textit{Bottom Row}: Response to small step disturbances at node 8,10,12 entering at time 2,6,10, respectively.The proposed blending controller not only stabilizes under saturation but also recovers the performance objective of rejecting small step disturbances. This contrasts against the non-integral controller, which sacrifices small-signal performance for stability. 


==> [ACC2020] Saturation_Arxiv_ver/windup_v1.tex <==
 We have showed  that projection nonlinearity of the controller \eqref{eq:NL-map} provides simple and effective solution to the constrained LQR problem when disturbance is known to be bounded. Now consider a linear input saturated system where the disturbances and initial condition are not necessarily constrained to have a known norm bound:
\begin{align}
\label{eq:lin-sat}
x_{t+1} = Ax_t+ \sat(u_t,u_{max}) + w_t
\end{align}
where the saturation nonlinearity is applied element-wise to the vector $u_t$.
In this scenario, controller $\SL{\CLM{x}}{\CLM{u}}$ previously constructed with \eqref{eq:NL-map} \textit{no longer} realizes the designed CLMs \eqref{eq:NL-map} for \eqref{eq:lin-sat}. Rather, the internal dynamics of \eqref{eq:lin-sat} with $\SL{\CLM{x}}{\CLM{u}}$ can be checked to be:
\begin{align}
\label{internal}
\hat{w}_t = A(\hat{w}_{t-1}-\p{max}{\hat{w}_{t-1}}) + w_{t-1}
\end{align}
 Nevertheless, we would like the saturated system to degrade gracefully and preserve stability. Such property is traditionally achieved via anti-windup design\cite{hu2008anti}. Here, we show that the proposed nonlinear controller achieves natural anti-windup property. 
\begin{lem}
If $A$ is schur, then internal dynamics \eqref{internal} is BIBO-stable. Further, if $\|A\|_{p} < \lambda <1 $, then $\limsup_{t \rightarrow \infty} \|\hat{w}_t\|_{p} < \frac{1}{1-\lambda} \|\b{w}\|_{p}$ with $p \in \{1,\infty\}$
\end{lem}
\begin{proof} Omitted in the interests of space
	\end{proof}
Similar to the large-scale constrained LQR case, since the "anti-windup" controller for the saturated linear system \eqref{eq:lin-sat} is composed of linear CLMs synthesized from \eqref{eq:S2} without the state constraint \eqref{eq:safety-1}, as will be illustrated in \secref{sec:sim}, distributed controller constraints can be easily incorporated. Thus, the given nonlinear controller can be considered as a distributed anti-windup controller. 


%
%
%\subsection{old version}
%Thus far, we have shown
%
%
%A related and natural question to ask is whether such control strategy works for saturated systems. It is plausible that the projection nonlinearity provides natural anti-windup property where finite-gain stability of the closed-loop is preserved and the system recovers linear scheme quickly under saturation. Further, if the controller is anti-windup, will the distributed properties discussed in \secref{sec:ls-lqr}? The answers to these questions are affirmative.\todo[inline]{the last two sentences are weird, needs rephrasing} Since our framework seeks explicit operators that map disturbance to states, the following is immediate.
%\begin{lem}
%\label{lem:finite-gain}
%Given a linear system with actuation saturation that has zero initial condition, \textit{i.e}, $x_0 = 0$:
%\begin{align}
%\label{eq:lin-sat}
%    x_{k+1} = Ax_k + \text{sat}_{u_{max}}(u_k) + w_k
%    \end{align}
% and a bound on disturbance such that $\|\b{w}\|_{\infty} \leq \eta_{max}$, 
%the closed loop under a controller of the form \eqref{eq:n-blend} with saturation projection constructed from CLMs synthesized in \eqref{eq:S2} without state constraints has finite-gain stability for all admissible $\b{w}$:
%$$\|\b{x}\| \leq \gamma \|\b{w}\|$$
%where $\gamma = \sum_{i = 1}^N (\eta_i - \eta_{i-1})\|R^{(i)}\|$
%\end{lem}
%\todo[inline]{Should be inf-norm, right?}
%\begin{proof}
%Application of norm submultiplicativity gives the finite gain bound.
%\end{proof}
%
%\begin{lem}\label{thm:antiwinduplqr}
%Consider the same conditions in \lemref{lem:finite-gain}, if $A$ is schur, then there exists $\gamma >0$ such that for all $\b{w}\in \ell_{2}$, 
%$$\|\b{x}\|_{2} \leq \gamma \|\b{w}\|_{}.$$
%\end{lem}
%\begin{proof}
%Omitted in the interest of space.
%\end{proof}
%\todo[inline]{Do you require also $\|w\|_{\infty} \leq \eta_{max} $? you said same conditions.. also norms are missing }
%
%% \begin{thm}\label{thm:antiwinduplqr}
%%  Assume that $\SL{\CLM{*x}}{\CLM{*u}}$ is applied to the linear system with input saturation  of the form $$x_{k+1} = Ax_k + \text{sat}_{u_{max}}(u_k) + w_k.$$
%% Then, if $A$ is marginally stable, then $\b{x}$ and $\b{u}$ are bounded for any bounded $\b{w}$.
%% \end{thm}
%% \begin{proof}
%% Omitted in the interest of space.
%% \end{proof}
%



==> blend_v1.tex <==
% \subsection{LTI System Level Approach}
% \noindent For a linear system $$ x_{t+1} =  Ax_t + B u_t + w_t, $$
% \cite{slsacc} has shown that for any matrices $R_k, M_k$ that satisfy the affine constraints
% \begin{subequations}
% \label{eq:lin-feaibility}
% \begin{align}
%     R_{1} &= I \\
%     R_{k+1} &= A R_k + B M_k, \quad k\leq T-1 \\
%     0 &= A R_T + B M_T, 
% \end{align}
% \end{subequations}

%\todo[inline]{Ideally the above Intro starts from linear sls and says that we have this relationship between closed loop maps and realizing controllers.. Then just say that we have way to extend this realtionship for general causal systems (ref to other paper)...and then say that here we will only focus on a particular type of nonlinear extension that helps for large-scale linear saturated systems }

%\subsection{Nonlinear SLS for Linear Input-Saturated System}
%\noindent Consider the linear system with input saturation
%\begin{align}\label{eq:linsat}
%    x_{k+1} = Ax_k + B \mathbf{Sat}(u_k) + w_k
%\end{align}
%We are proposing the following system level controller implementation 
%\begin{subequations}
%\begin{align}
%\label{eq:nl-controller-1}
%    \hat{w}_t &= x_t - \sum^{N}_{i=1}\sum^{T-1}_{k=1}R^{i}_{k+1}G^i(\hat{w}_{t-k})\\
%    \label{eq:nl-controller-2} u_t &= \sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(\hat{w}_{t-k})
%\end{align}
%\end{subequations}
%parametrized by matrices $R^i_k$ and $M^i_k$ that satisfy:
%%\begin{subequations}
%%\label{eq:lin-feaibility}
%%\begin{align}
%%    R^i_{1} &= I \\
%%    R^i_{k+1} &= A R^i_k + B M^i_k, \quad k\leq T-1 \\
%%    0 &= A R^i_{T} + B M^i_{T}, 
%%\end{align}
%%\end{subequations}
%and some nonlinear maps $G^{i}$. A crucial design principle will be that the maps $G^{i}$ are chosen such that the controller never enters the saturated regime:
%\begin{asp}\label{asp:G}
%Assume $G^{i}( \cdot )$ are chosen such that for all $z_1$, $\dots$, $z_T$ holds:
%$$\mathbf{Sat}\left(\sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(z_k)\right) = \sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(z_k)$$
%\end{asp}
%Now, given our design assumption \aspref{asp:G} substituting the dynamics \eqref{eq:linsat} in \eqref{eq:nl-controller-1} and then using the same expressions \eqref{eq:nl-controller-1}, \eqref{eq:nl-controller-2} to express $x_{t-1}$ and $u_{t-1}$ in terms of  $\hat{w}_{t-k}$, $1 \leq k \leq T$, we get the following equation for the dynamics of $\hat{w}_t$:
%\begin{align}
%   \hat{w}_{t+1} &= A(\hat{w}_t - \sum^{N}_{i=1} G^i(\hat{w}_{t})) + w_{t}
%\end{align}
%We will refer to the internal state $\hat{w}_t$ as the \textit{effective disturbance}. If we have stability for $\hat{w}_t$, the relation \eqref{eq:nl-controller-1} and \eqref{eq:nl-controller-2} show that we also imply stability for the state $x$ and input $u$, since 
%\begin{align*}
%    x_t &= \hat{w}_t + \sum^{N}_{i=1}\sum^{T-1}_{k=1}R^{i}_{k+1}G^i(\hat{w}_{t-k})\\ u_t &= \sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(\hat{w}_{t-k})
%\end{align*}
%
%For this paper we will choose 
%\begin{align}
%    G^i(w) = \p{i}{w}-\p{i-1}{w}
%\end{align}
% where $\p{i}{w}$ denote different projection operators. Correspondingly, the dynamics of  \eqref{eq:intDyn} then become 
% \begin{align}
%     \label{eq:intDyn2}
%   \hat{w}_{t+1} &= A(\hat{w}_t - \p{N}{\hat{w}_t}) + w_{t}
% \end{align}

As introduced in the previous section, system level controllers defined in \defref{def:SL} can implement arbitrary CLM for causal nonlinear systems of the form \eqref{eq:sys}. The results in \cite{NLSLSHODoyle2019} motivate a new approach for nonlinear control synthesis: Searching for stable operators $\TX$, $\TU$ that are CLMs satisfying \eqref{eq:feasnl} and constructing a corresponding system level controller $\SL{\TX}{\TU}$ by \defref{def:SL}.

It is conceivable that the generality of this approach could lead to an entirely new direction of nonlinear dynamic control methods. Serving as a first step towards exploring the potential of this new perspective, the remainder of this paper focuses on a subset of nonlinear system level controllers $\SL{\TX}{\TU}$ that proves particularly useful for controlling large-scale linear systems subject to state/input constraints and input saturation.

%In particular we will restrict ourselves to the class of controllers $\SL{\TX}{\TU}$ where $\TX$ and $\TU$ are structured as
%
%Here $G^{i}, i\in \set{N}$ are to-be-designed nonlinear functions.  $R^{(i)}_k \in \RR^{n\times n}$, $M^{(i)}_k \in \RR^{p\times n}$ are matrices associated with linear FIR CLM $\CLM{x,i}$,$\CLM{u,i}$, $i \in \set{N}$ of horizon $T$ for a linear system of interests: 
%\begin{align} \label{eq:syslin}x_{k+1} =Ax_k + Bu_k + w_k \end{align}
%such that for each $i \in \set{N}$, $\CLM{x,i}$,$\CLM{u,i}$ satisfies \eqref{eq:lin-feaibility}.  The dynamic controller \eqref{eq:SLeq} that achieves \eqref{eq:n-blend} has the following explicit form:
%\begin{subequations}
%	\begin{align}
%	\label{eq:nl-controller-1}
%	\hat{w}_t &= x_t - \sum^{N}_{i=1}\sum^{T-1}_{k=1}R^{i}_{k+1}G^i(\hat{w}_{t-k})\\
%	\label{eq:nl-controller-2} u_t &= \sum^{N}_{i=1}\sum^{T-1}_{k=0}M^{i}_{k+1}G^{i}(\hat{w}_{t-k}).
%	\end{align}
%\end{subequations}
%\todo[inline]{The internal dynamics part is missing... you say the dynamic controller achieves the CLMs but that's not true, because if you don't choose $\Sigma_i G^i = I$, then 14a and 14b are not realizable CLM's only approximate ones..}


In particular we will restrict ourselves to the class of controllers $\SL{\TX}{\TU}$ where $\TX$ and $\TU$ are structured as
\begin{subequations}
	\label{eq:n-blend}
	\begin{align}
	% \clm{x}{t}(w_{t-1:t-T}) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}R^{(i)}_{k} (\p{i}{w_{t-k}}-\p{i-1}{w_{t-k}} )\\
	\clm{x}{t}(\cdot) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}R^{(i)}_{k}  (\p{i}{w}-\p{i-1}{w})\\
	\clm{u}{t}(\cdot) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}M^{(i)}_{k}( \p{i}{w}-\p{i-1}{w}).
	\end{align}
\end{subequations}

We choose $\eta_N\geq\eta_{N-1}\geq \dots \geq \eta_0 =  0$ and  the operator $\p{i}{\cdot}:\RR^{n} \rightarrow \RR^n$ as any nonlinear function with a projection-like property defined for parameter $\eta_i$. $R^{(i)}_k \in \RR^{n\times n}$, $M^{(i)}_k \in \RR^{p\times n}$ are matrices associated with linear FIR CLMs $\CLM{x,i}$,$\CLM{u,i}$, $i \in \set{N}$ of horizon $T$ for a linear system of interests: 
\begin{align} \label{eq:syslin}x_{k+1} =Ax_k + Bu_k + w_k \end{align}
with $x_t \in \RR^n$,$w_t \in \RR^n$, $u \in \RR^p$ such that for each $i \in \set{N}$, $\CLM{x,i}$,$\CLM{u,i}$ satisfies \eqref{eq:lin-feaibility}.
 Concretely, we consider two specific nonlinear projections:
 
 \begin{defn}[Saturation Projection]\label{def:sat}
 	Let vector $w = [w^1, \dots, w^n]^T$. The saturation projection is an element-wise projection:\begin{align}
 	\p{}{w}:= \begin{bmatrix}
 	\sat(w^1,\eta)\\ \vdots\\
 		\sat(w^n,\eta)
 	\end{bmatrix}
 	\end{align}
 	where $\sat(w,\eta) = \text{sign}(w) \max\{|w|,\eta\}$.
 \end{defn}

\begin{defn}[Radial Projection] \label{def:radial}
The radial projection is defined as:\begin{align}
    \p{}{w}:= \frac{\sat(\|w\|_{\infty}/\eta,1)}{\|w\|_{\infty}/\eta} w
\end{align}
\end{defn}


Unless otherwise specified, the results derived in the rest of the paper hold for both projections.
%\begin{rem}
% For $n=1$, radial projection and saturation projection coincide with each other. The radial and saturation projection operator act as the identity whenever $\|w\|_{\infty} \leq \eta$. Otherwise, the radial projection rescales $w$ such that $\|\p{}{w}\|_{\infty} = \eta$ whereas the saturation projection performs element-wise radial projection.
%\end{rem}


The proposed nonlinear controller $\SL{\CLM{x}}{\CLM{u}}$ can be thought of as a \textit{nonlinear blend} of the \textit{linear} FIR controllers $\SL{\CLM{x,i}}{\CLM{u,i}}$, $i \in \set{N}$. Although the nonlinear operator $\CLM{x}$, $\CLM{u}$ differs from its linear components $\CLM{x,i}$, $\CLM{u,i}$ only by the static nonlinear function $\p{i}{w}$, the upcoming sections will demonstrate that this simple additional nonlinearity proves surprisingly useful. In particular, $\eta_i$'s separate any disturbance $w_t$ into $N$ zones such that for each $i$th linear controller $\SL{\CLM{x,i}}{\CLM{u,i}}$, only the portion of $w_t$ that "falls" between $\eta_i$ and $\eta_{i-1}$ is acted upon. Intuitively, one could choose different behaviours for various portions of the disturbance signal, specifying either performance or safety properties.





For ease of exposition, we focus on the two-zone case of the proposed controller $\SL{\CLM{x}}{\CLM{u}}$ though all the analysis extends naturally to the $N$-zone case. 
Thus, \eqref{eq:n-blend} simplifies to
\begin{align}
    \clm{x}{t}(w_{t-1:0}) = \sum^{\min\{T,t\}}_{k=1} &\R1{k} \p{1}{w_{t-k}} + \label{eq:NL-map}\\
    & \R2{k}(\p2{w_{t-k}} - \p1{w_{t-k}}) \nonumber \\
    \clm{u}{t}(w_{t-1:0}) = \sum^{\min\{T,t\}}_{k=1} &\M1{k} \p{1}{w_{t-k}} +\nonumber \\
    & \M2{k}(\p2{w_{t-k}} - \p1{w_{t-k}}). \nonumber\label{eq:NL-map-2}
\end{align}
% The operators $\TX$, $\TU$ are nonlinear due to the nonlinearity introduced by the projection $\p{}{w}$. Nevertheless, by plugging equation \eqref{eq:NL-map} into the general CLM conditions of \thmref{thm:sufnec}, it can be verified that $\TX$, $\TU$ are nonlinear CLMs of the linear system \eqref{eq:syslin} for small disturbances. This is summarized in the next lemma:
% \begin{lem}
% If $\{\CLM{x,i}$,$\CLM{u,i}\}_{i = 1,2}$ are CLM for \eqref{eq:syslin}, then the nonlinear operators $\TX$, $\TU$ defined in \eqref{eq:NL-map} are CLMs of \eqref{eq:syslin} for all $\b{w}$ that satisfy $\sup_k \|w_k\|_{\infty} \leq \eta_2$.
% \end{lem}
Note that system level controller $\SL{\CLM{x}}{\CLM{u}}$ of the two-zone CLM is internally stabilizing and achieves the two-zone CLM behaviour for \eqref{eq:syslin}  as long as $\|\b{w}\|_{\infty} \leq \eta_2$ with $x_0 = 0$. 
% The closed loop dynamics simplify to:
% \begin{subequations}
% \label{eq:cleq_blend}
% \begin{align}
%   \label{eq:clint_blend} 
%   \hat{w}_{t+1} &= A(\hat{w}_t-\p{2}{\hat{w}_t}) + w_t\\
%     \label{eq:clx_blend}    
%     x_t &= \Tx{t}\left(0,0,\hat{w}_{t-1:1}\right)+\hat{w}_{t}\\
%     \label{eq:clu_blend}u_t &= \Tu{t}\left(0,\hat{w}_{t:1}\right)
% \end{align}
% \end{subequations}

% \begin{rem}
% The blending of \textit{two} linear CLM in \eqref{eq:NL-map} can be naturally extended to \textit{$N$} linear CLM by extending \eqref{eq:NL-map} to the form:
% \begin{align}\label{eq:blend}
% \clm{x}{t}(w_{t-1:t-T}) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}R^{(i)}_{k} \p{i}{w_{t-k}} \\
% \clm{u}{t}(w_{t-1:t-T}) &= \sum^{N}_{i=1} \sum^{\min\{T,t\}}_{k=1}R^{(i)}_{k} \p{i}{w_{t-k}} 
% \end{align}
% where $R^{(i)}_{k}$, $M^{(i)}_{k}$ are matrices associated with $N$ linear FIR CLM $\CLM{x,i}$, $\CLM{u,i}$.
% \end{rem}

In the remainder of this paper we will explore the consequence of this blending technique for decentralized control design with respect to input saturation and state constraints in linear systems. It will become clear that with the simple projection nonlinearity, \eqref{eq:NL-map} offers a variety of advantages over linear controllers.

==> intro_v1.tex <==


In this paper, we propose a novel offline distributed nonlinear controller synthesis procedure that outperforms any optimal linear controller for constrained LQR problem \cite{maciejowski2002predictive, zhang2013distributed,li2011disturbance,SLSChenAnderson2019}. In addition, the same controller inherently prevents windup-instabilities in saturated linear systems which are traditionally mitigated via additional anti-windup design \cite{kothare1994unified, kolmanovsky2014reference,hu2008anti}. Another significant advantage of the approach, is that despite being a nonlinear synthesis method it naturally enjoys the same benefits as the linear system level approach introduced in \cite{anderson2019system}, which makes it scalable in the large-system setting. 

 Our work is largely based on \cite{NLSLSHODoyle2019}, which describes the system-level characterization of closed loops of general nonlinear discrete-time systems. Moreover, \cite{NLSLSHODoyle2019} introduces a simple universal control structure, called a system level controller, that has the capacity to stabilize any nonlinear system if parametrized with the according closed loop maps. In this paper, we will show that just using a very special case of the framework presented in \cite{NLSLSHODoyle2019} provides new promising tools for control design. In particular, we will illustrate how a simple projection nonlinearity can become a powerful tool for solving the problems described above. 

 
The rest of the paper starts with a review on nonlinear System Level Synthesis (NLSLS) in \secref{sec:nlsls}. The proposed nonlinear controller is introduced in \secref{sec:blend}, followed by \secref{sec:lqr} where the constrained LQR problem is discussed. We show in \secref{sec:ls} that the proposed nonlinear controller has natural anti-windup properties and therefore allow for large-scale distributed design. Numerical simulation in \secref{sec:sim} validates the presented theory. 

==> lqr_v1.tex <==
We present a novel nonlinear controller synthesis procedure for a class of constrained LQR problems using the proposed SL controller with CLMs \eqref{eq:NL-map}. In particular, we will show that the synthesized  nonlinear blending system level controller is guaranteed to outperform any linear controller for the class of constrained LQR problems to be discussed. Additionally, we comment on how structural constraints for large-scale systems such as delay, actuation sparsity, and localization can be easily accommodated for our nonlinear controller. 

\subsection{Problem Statement}
% Consider a linear quadratic optimal control problem where system disturbances are mostly small but  occasionally large enough to cause input or state constraint violation, which we shall dub as safety constraints.
Consider a control problem where we wish to minimize an \textit{average} LQR cost, but also want that the closed loop meets certain safety guarantees against a set of rare yet possible \textit{worst-case} disturbances. Ideally, we would like to synthesize a controller that can guarantee the necessary safety constraints without too much loss in performance compared to the unconstrained LQR controller.

We will phrase this design goal as the following constrained LQR problem:
\begin{subequations}
\label{eq:const-lqr}
\begin{align}
\label{eq:cost-lqr}&\min_{\b{K}}\lim_{T \rightarrow \infty}\frac1T \sum_{t=1}^T \mathbb{E}_{w_t^i \sim p(w)}[\mathcal{J}(x_t,u_t) ] \\
&s.t.\,\,\,\,\,\,\,\,\,\,\,\, x_{t+1} = Ax_{t}+Bu_t + w_t\label{eq:lin-dyn}\\
 &\qquad  \,\,\,\,\,\,\,\,\,\,\,\,\,\,\,u_t = \b{K}(x_{t:0})\\
 & \qquad \forall \b{w}: \sup_k||w_k||_{\infty}\leq \eta_{max}:  \\
\label{eq:XUconstlqr}&\,\,\,\,\,\,\,\,\,\,\,\,\,\qquad  \sup_k ||x_k||_{\infty}\leq x_{max} \quad \sup_k ||u_k||_{\infty}\leq u_{max}  \nonumber
% \\
%\label{eq:Uconstlqr}&\,\,\,\,\,\,\,\,\,\,\,\,\, \qquad  \sup_k ||u_k||_{\infty}\leq u_{max} 
\end{align}
\end{subequations}
where $\mathcal{J}$ abbreviates the quadratic stage cost $\mathcal{J}(x,u) = x^TQx+uPu$ with $Q$,$P \succ 0$. Moreover, we will assume that the disturbance is stochastic but bounded and satisfies $\|w_k\|_{\infty} \leq \eta_{max}$ for all time $k$. Let the distribution of the disturbance be known and for ease of exposition, we will make the following additional assumption:
\begin{asp}
\label{assum:distribution}
Disturbance $w_t^i$ are i.i.d. drawn from the scalar centered distribution $p(w)$ and uncorrelated in time $t$ and coordinate $i$.
%$$ \E [w_t^i w_{t'}^j] = 0  \quad \forall i\not = j, t\not = t'$$
% In addition, we assume a bound on $w_k^i$, $\forall k,i$ such that $||w_k^i||\leq \eta_2$.
\end{asp}
More formally, we can use the system level framework introduced in \secref{sec:nlsls} to write the optimal control problem \eqref{eq:const-lqr} equivalently as an optimization over all characterizing CLMs $\CLM{x}$ and $\CLM{u}$ of the dynamics by recalling \thmref{thm:sufnec}:
\begin{subequations}
\label{eq:const-lqrclm}
\begin{align}
\label{eq:cost-lqrclm-cost2}&\min_{\CLM{x},\CLM{u}}\lim_{T \rightarrow \infty}\frac1T \sum_{t=1}^T \mathbb{E}[\mathcal{J}(\clm{x}{t}(w_{t:0}),\clm{u}{t}(w_{t:0})) ]
 \\
\label{eq:const-lqrclm-constclm2} &s.t. \,\,\, \,\,\,\,\,\,\,\, \clm{x}{t}(w_{t:0}) = \clm{x}{t}(0,0,w_{t-2:0}) + w_{t-1} \\
\nonumber&\clm{x}{t+1}(0,0,w_{t-1:0}) = A\clm{x}{t}(0,w_{t-1:0})+B\clm{u}{t}(0,w_{t-1:0})\\
 \label{eq:const-lqrclm-constx2} &\qquad \forall t, \|w_t\|_{\infty} \leq \eta_{max}:\quad \|\clm{x}{t}(w_{t:0})\|_{\infty} \leq x_{\mathrm{max}} \\
  \label{eq:const-lqrclm-constu2} &\qquad \forall t, \|w_t\|_{\infty} \leq \eta_{max}:\quad \|\clm{u}{t}(w_{t:0})\|_{\infty} \leq u_{\mathrm{max}} 
\end{align}
\end{subequations}
% \begin{subequations}
% \label{eq:const-lqrclm}
% \begin{align}
% \label{eq:cost-lqrclm-cost}&\min_{\b{K}}\lim_{T \rightarrow \infty}\frac1T \sum_{t=1}^T \mathbb{E}_{w_t^i \sim p(w)}[\mathcal{J}(\clm{x}{t}(w_{t:0}),\clm{u}{t}(w_{t:0})) ] \\
% \label{eq:const-lqrclm-constclm} &s.t.\,\,\, \CLM{x} = \CLMofFK{x}{Ax+Bu}{\b{K}},\quad \CLM{u} = \CLMofFK{u}{Ax+Bu}{\b{K}}\\
%  \label{eq:const-lqrclm-constx} &\qquad \forall t, \|w_t\|_{\infty} \leq \eta_{2}:\quad \|\clm{x}{t}(w_{t:0})\|_{\infty} \leq x_{\mathrm{max}} \\
%   \label{eq:const-lqrclm-constu} &\qquad \forall t, \|w_t\|_{\infty} \leq \eta_{2}:\quad \|\clm{u}{t}(w_{t:0})\|_{\infty} \leq u_{\mathrm{max}} 
% \end{align}
% \end{subequations}
% Furthermore,

As in the linear SLS case \cite{anderson2019system}, we do not need to have the controller $\b{K}$ be a decision variable, since we can always realize the optimal solution $\{\b{\Psi}^{(x)*},\b{\Psi}^{(u)*}\}$ to \eqref{eq:const-lqrclm} with a system level controller $\SL{\b{\Psi}^{(x)*}}{\b{\Psi}^{(u)*}}$.
% For the rest of the paper, we further assume weighting matrices $Q$ and $R$ to be identity to avoid overloading notation.
% Consider scenarios where the disturbances are mostly small but occasionally large enough to cause input or state constraint violation, which we shall dub as safety constraints. One naturally would wish to minimize the \textit{average} LQR cost while ensure safety constraints against the \textit{worst-case} albeit \textit{infrequent} disturbance. When disturbances are not adversarial and rarely achieve the worst-case norm, the controller synthesis procedure should exploit such knowledge. We capture this intuition by assuming disturbances are drawn from a centered distribution, $p(w)$ with bounded support. Without loss of generality, we make the assumption about disturbance below for simplicity of exposition. Note that the upcoming analysis can be carried out without it:
% \begin{asp}
% \label{assum:distribution}
% Disturbance $w_k^i$ are i.i.d. drawn from the scalar distribution $p(w)$ and uncorrelated in time and location, \textit{i.e.},
% $$ \E [w_t^i w_{t'}^j] = 0  \quad \forall i\not = j, t\not = t'$$
% In addition, we assume a bound on $w_k^i$, $\forall k,i$ such that $||w_k^i||\leq \eta_2$.
% \end{asp}

% Denote the LQR stage cost $\mathcal{J}_t(x_t,u_t) = x_t^TQx_t+u_tPu_t$, we aim to solve the following constrained LQR problem:
% \begin{subequations}
% \label{eq:const-lqr}
% \begin{align}
% \label{eq:cost-lqr}\min_{\b{K}} &\lim_{T \rightarrow \infty}\frac1T \sum_{t=1}^T \mathbb{E}_{w_t^i \sim p(w)}[\mathcal{J}_t(x_t,u_t) ] \\
% s.t.&\,\,\,\,\,\,\,\,\,\,\,\, x_{t+1} = Ax_{t}+Bu_t + w_t\label{eq:lin-dyn}\\
%  &\qquad  \,\,\,\,\,\,u_t = \b{K}(x_{t:0})\\
% & \forall w_k\text{ , } \forall k \in \mathbb{N}:  \left\|w_k \right\|_{\infty} \leq \eta_2 \text{ , }  \nonumber\\
% \label{eq:Xconstlqr}& \quad ||x_k||_{\infty} \leq x_{max} \quad \forall k\\
% \label{eq:Uconstlqr}& \quad  ||u_k ||_{\infty} \leq u_{max} \quad \forall k
% \end{align}
% \end{subequations}

% To avoid overloading notations, we also adopt the following assumption:
% \begin{asp}
% \label{assum:C+D}
% $Q = I$ and $P = I$.
% \end{asp}
% We aim to synthesize nonlinear  controller for a large scale linear systems with input and state constraints. The input constraints are assumed to be decentralized saturation-type constraints such that $\|u_t\|_{\infty}\leq u_{max}$ and the state constraints to be $\|x_t\|_{\infty}\leq x_{max}$\footnote{General polytopic input and state constraints can be similarly considered as in the sequel.}.



% Often the disturbances are mostly small, but occasionally large enough to cause safety violation. Therefore it is natural to have different control objectives depending on if we are facing small disturbances or large disturbances:
%  \begin{itemize}
% \item  (O1): If $w_k$ is small such that state constraint is guaranteed and input saturation does not happen, we want to prioritize performance with a \textit{performance-oriented} control strategy.
% \item (O2): If $w_k$ is large, we want to control in a \textit{safety-oriented} fashion by enforcing the input and state constraints. 
% \end{itemize}  


% For example, $p(w)$ could be multivariate truncated Gaussian distribution with estimated variance.
\subsection{Conservativeness of Linear Solutions}\label{sec:linneg}
We will first discuss properties of solutions to our original problem \eqref{eq:const-lqr}, if we restrict ourselves to only linear controllers $\b{K}$. As shown previously we can consider the equivalent problem formulation \eqref{eq:const-lqrclm}, where we restrict the CLMs $\{\CLM{x},\CLM{u}\}$ to be linear. This poses a convex problem and as shown in \cite{SLSChenAnderson2019}, it can be solved by searching over FIR CLMs $\{\CLM{x},\CLM{u}\}$ with large enough horizon $T$ and a realizing controller is $\SL{\CLM{x}}{\CLM{u}}$. Yet, the corresponding linear optimal CLMs $\{\CLM{x,lin*},\CLM{u,lin*}\}$ come with undesirable restrictions:

\begin{itemize}
    \item $\{\CLM{x,lin*},\CLM{u,lin*}\}$ impose stricter safety constraints than the required constraints \eqref{eq:const-lqrclm-constx2} and \eqref{eq:const-lqrclm-constu2}. 
    \item $\{\CLM{x,lin*},\CLM{u,lin*}\}$ do not depend on the disturbance distribution $p(w)$. 
\end{itemize}

To see the first point, we have the following result as a consequence of linearity:
\begin{lem}
For any linear $\{\CLM{x,lin},\CLM{u,lin}\}$, the constraint \eqref{eq:const-lqrclm-constx2},\eqref{eq:const-lqrclm-constu2} is equivalent to
\begin{subequations}
\label{eq:strict}
\begin{align}
\sup_t \|\clm{x,lin}{t}(w_{t:0})\|_{\infty} &\leq \sup_t \|w_t\|_{\infty} \frac{x_{max}}{\eta_{max}}\\
\sup_t \|\clm{u,lin}{t}(w_{t:0})\|_{\infty} &\leq \sup_t \|w_t\|_{\infty} \frac{u_{max}}{\eta_{max}}
\end{align}
\end{subequations}
\end{lem}
\begin{proof}
Clearly, \eqref{eq:strict} implies \eqref{eq:const-lqrclm-constx2},\eqref{eq:const-lqrclm-constu2}. The reverse implication follows by the assumed linearity of $\{\CLM{x,lin},\CLM{u,lin}\}$ and homogeneity of norms.
\end{proof}
To elaborate on the second point, notice that for linear CLMs $\CLM{x,lin},\CLM{u,lin}$ our objective function \eqref{eq:cost-lqrclm-cost2} can be expressed equivalently as 
\begin{align}\label{eq:H2simplify}
    \eqref{eq:cost-lqrclm-cost2} = \sigma^2\left\|\begin{array}{c}Q^{1/2} \CLM{x}\\ P^{1/2}\CLM{u} \end{array} \right\|^2_{\mathcal{H}_2},\quad \sigma^2:=\E_{w \sim p(w)}[w^2]
\end{align}
where $\sigma^2$ denotes the variance of the scalar distribution $p(w)$ and $\|.\|_{\mathcal{H}_2}$ denotes the $\mathcal{H}_2$ norm for linear operators. Since the objective function only gets scaled by a constant factor $\sigma^2$ for different distributions $p(w)$, this shows that for linear CLMs, the solutions $\{\CLM{x,lin},\CLM{u,lin}\}$ to \eqref{eq:const-lqrclm} are independent of the distribution $p(w)$. 

% To elaborate on the second point, we first note that the optimal solution to \eqref{eq:const-lqr} can be equivalently recovered by solving for the optimal linear CLM to \eqref{eq:lin-dyn}. Applying \assref{assum:distribution} and casting objective function \eqref{eq:cost-lqr} in terms of linear CLM of the form \eqref{eq:linear-maps} where $\b{x} = \b{R}\b{w}$ and ,$\b{u} = \b{M}\b{w}$ with $\b{R} = [R_1, R_2,\dots]$ and $\b{M} = [M_1, M_2,\dots]$ the linear operator, we have:
% \begin{align}
% \eqref{eq:cost-lqr}= 
% \E[(w_t^i)^2] \cdot \Trace  \left( \b{R}^T\b{R} +  \b{M}^T\b{M}  \right) 
% \end{align}

%In summary, a linear approach to problem \eqref{eq:const-lqr} not only has the drawback that the resulting closed loop will enforce safety constraints that are too conservative, but will completely ignore knowledge of the disturbance $p(w)$ during synthesis. In contrast, in many applications the disturbance can be assumed to be mostly small and only occasionally achieve worst-case size and it is conceivable that there should be a way to exploit this knowledge for control synthesis.


% We will see that especially when the variance of the disturbance is small, the optimal blended controller can offer a big improvement over linear optimal controllers.

%As we will see in the later sections, due to the former restrictions a linear controller will act to 
% Since solving the constrained LQR problem without expectation over $w$ is the same as solving one with given $p(w)$, the information about distribution is lost in the optimization over linear $\b{K}$ due to linearity.
% \begin{subequations}
% \label{eq:const-sls}
% \begin{align}
% \label{eq:costsls}\min_{\{\R1{k},\M1{k}\}_{k = 1:T}} &  \E[(w_t^i)^2] \cdot \Trace  \left( \begin{bmatrix} \R1{T:1} \\ \M1{T:1} \end{bmatrix} \begin{bmatrix} \R1{T:1} \\ \M1{T:1} \end{bmatrix}^T  \right)  \\
% s.t.&\,\,\,\,\,\,\,\,\, R_{k+1} = AR_{k} + BM_k \label{lin-sls-1}\\
% &\,\,\,\,\,\,\,\,\, R_{1} = I\label{lin-sls-2}\\
% &\,\,\,\,\,\,\,\,\, R_{T} = 0\label{lin-sls-3}\\
% & \forall w_k, k = 1,\dots,T,  \text{ with }  \left\|w_k \right\|_{\infty} \leq \eta: \nonumber\\
% \label{eq:Xconstsls}& \quad ||\sum_{k = 0}^{T-1} R_k w_{T-k}||_{\infty} \leq x_{max} \\
% \label{eq:Uconstsls}& \quad  ||\sum_{k = 0}^{T-1} M_k w_{T-k} ||_{\infty} \leq u_{max}
% \end{align}
% \end{subequations}
% To see the equivalence, note that \eqref{lin-sls-1}-\eqref{lin-sls-3} are the feasibility test for FIR linear CLM $\{\R1{k},\M1{k}\}_{k = 1:T}$. 


% We will refer to the above linear SLS constrained LQR problem as $\pro{\eta}$ since the solutions will have different properties depending on the value of $\eta$. On the one extreme, the centralized and distributed solution with $\eta=\eta_2$ was given in \cite{SLSChenAnderson2019} but we are optimizing for the worst-case performance. We call the solution to $\pro{\eta_2}$ the safe controller. On the other extreme, if we choose $\eta=\epsilon$ for small $\epsilon$, then  we will essentially obtain the optimal SLS controller as detailed in \cite{wang2019system} without the constraints \eqref{eq:Xconstsls} and \eqref{eq:Uconstsls} for (O1).

% Nevertheless, we would not like the apply either of the two. As will be demonstrated in \secref{sec:sim}, performance (as measured by the optimal LQR cost degradation) caused by conservatism can result in a big gap between unconstrained optimal controller performance and safe controller performance.
% The above discussion calls for a control strategy that offers flexibility depending on the size of disturbance. Ideally, the controller could take advantage of small disturbance and prioritize performance while being conservative when disturbance becomes larger information. 

\subsection{A NLSLS Take}
\label{sec:nlsls-take}
% Consider the general problem \eqref{eq:const-lqrclm2}
% Here we will show that the proposed nonlinear blend controller \eqref{eq:NL-map}

% the general problem \eqref{eq:const-lqrclm2} \eqref{eq:NL-map}
Consider the general problem \eqref{eq:const-lqrclm}, where now we search over CLMs $\{\CLM{x},\CLM{u}\}$ of the form presented in \eqref{eq:NL-map} with the choice of $\eta_2= \eta_{max}$, some $\eta_1<\eta_2$, and a finite memory horizon $T$. Recall that $\{\CLM{x},\CLM{u}\}$ is a blending of two linear CLMs and has the form \eqref{eq:NL-map}. Restricting ourselves to this form of CLMs, allows us to derive the following convex problem which is a relaxation of the general problem  \eqref{eq:const-lqrclm}:
% \begin{subequations}
% \label{eq:NL-map2}
% \begin{align}
%     \clm{x}{t}( w_{t:0}) = \sum^{\min\{T,t\}}_{k=1} &\R1{k} \p{1}{w_{t-k}} + \nonumber \\
%     & \R2{k}(\p2{w_{t-k}} - \p1{w_{t-k}}) \label{eq:NL-map-1}\\
%     \clm{u}{t}(w_{t:0}) = \sum^{\min\{T,t\}}_{k=1} &\M1{k} \p{1}{w_{t-k}} +\nonumber \\
%     & \M2{k}(\p2{w_{t-k}} - \p1{w_{t-k}}) \label{eq:NL-map-2}
% \end{align}
% \end{subequations}
% where $\{\R1{k}$, $\M1{k}\}_{k = 1:T}$ and $\{\R2{k}$, $\M2{k}\}_{k = 1:T}$ are the corresponding matrices of the linear CLMs $\{\CLM{x,1},\CLM{u,1}\}$ and  $\{\CLM{x,2}\CLM{u,2}\}$.
\begin{subequations}
\label{eq:S2}
\begin{align}
 \label{eq:cost-blend} \min_{\R{i}{}, \M{i}{}} & \left\|\begin{bmatrix} Q&0\\ 0 & P\end{bmatrix}^{1/2} \begin{bmatrix} \R1{} & \R2{} \\ \M1{}&\M2{}\end{bmatrix} \Sigma^{1/2}_w \right\|^{2}_{F}  \\
\label{eq:safety-1} 
s.t.\quad& \eta_1\|\R1{}\|_{\infty} + (\eta_2 - \eta_1)\|\R2{}\|_{\infty} \leq x_{max}\\
 &\eta_1\|\M1{}\|_{\infty} + (\eta_2 - \eta_1)\|\M2{}\|_{\infty} \leq u_{max} \label{eq:safety-2}\\
 & \R{i}{k+1} = A\R{i}{k} + B\M{i}k \label{lin-feas1}\\
 & \R{i}{1} = I,\quad \R{i}{T} = 0  \nonumber
\end{align}
\end{subequations}
where 
\begin{equation}
\label{eq:sigma} 
      \Sigma_w = \begin{bmatrix} \alpha_1 I & \alpha_2 I \\ \alpha_2 I &  \alpha_3 I  \end{bmatrix} \nonumber
    % \nonumber\\
    % \alpha_1 &= \E[\p1{w_t^i}^2]\nonumber \\
    % \alpha_2 &= \E[\p1{w_t^i} (\p2{w} -\p1{w_t^i})] \nonumber \\
    % \alpha_3 &= \E[(\p2{w_t^i} - \p1{w_t^i})^2] \nonumber\\
%       c_x &= ||[\R1T \R1{T-1} \R1{T-2} \dots \R11]||_{\infty}  \nonumber\\
%  c_u &= ||[\M1T \M1{T-1} \M1{T-2} \dots \M11]||_{\infty}   \nonumber
\end{equation}
with $\alpha_1 = \E[\p1{w}^2]$, $\alpha_2 = \E[\p1{w} (\p2{w} -\p1{w})]$, and $\alpha_3 = \E[(\p2{w} - \p1{w})^2]$, where $w \sim p(w)$. Moreover $\R{i}{}$ and $\M{i}{}$ are abbreviations for the row-wise concatenation of the matrices associated with the linear CLMs $\CLM{x,i}$, $\CLM{u,i}$, \textit{i.e}, $\R{i}{} = [\R{i}{T}, \R{i}{T-1}, \dots ,\R{i}{1}]$, $\M{i}{} = [\M{i}{T}, \M{i}{T-1}, \dots ,\M{i}{1}]$. Hereby, only constraints \eqref{eq:safety-1}, \eqref{eq:safety-2} are sufficient condition of the constraint \eqref{eq:const-lqrclm-constx2}, \eqref{eq:const-lqrclm-constu2} via norm multiplicativity. All other equations in the optimization are equivalent to the original optimization. Finally, solving the convex problem \eqref{eq:S2} gives us the sub-optimal nonlinear CLMs $\{\CLM{*x}, \CLM{*u}\}$ for the system dynamics \eqref{eq:lin-dyn}, which can be realized with the internally stabilizing system level controller $\SL{\CLM{*x}}{\CLM{*u}}$.
% Considering the following optimization over the linear CLM $\CLM{x,1}$,$\CLM{u,1}$ and $\CLM{x,2}$,$\CLM{u,2}$ for fixed $\eta_1 \in [0,\eta_2]$. Define row-wise concatenated matrices $\R{i} = [\R{i}{T}, \R{i}{T-1}, \dots ,\R{i}{1}]$, $\M{i} = [\M{i}{T}, \M{i}{T-1}, \dots ,\M{i}{1}]$
%Synthesis \eqref{eq:S2} jointly optimizes two linear CLM such that the nonlinear CLM \eqref{eq:NL-map2} still ensures the overall safety of the closed loop.
% The objective function \eqref{eq:cost-blend} is a \textit{equivalent} to the objective function of \eqref{eq:cost-lqrclm-cost2} by plugging \eqref{eq:NL-map2} into \eqref{eq:cost-lqr}. The safety constraint \eqref{eq:XUconstlqr} is relaxed through norm submultiplicativity to \eqref{eq:safety-1} and \eqref{eq:safety-2}. It is also straightforward to see that \eqref{eq:NL-map2} is an FIR CLM for dynamics \eqref{eq:lin-dyn} if and only if $\CLM{x,1}$,$\CLM{u,1}$,$\CLM{x,2}$,$\CLM{u,2}$ satisfy linear FIR CLM feasibility constraint \eqref{lin-feas1}-\eqref{lin-feas3}. 
%The nonlinear controller $\SL{\CLM{x}}{\CLM{u}}$ can then be constructed as a special case of \eqref{eq:SLeq} from the CLM synthesized in \eqref{eq:S2}:
% \begin{subequations}
% \label{eq:optimalblend}
% \begin{align}
%     \hat{w}_t &= x_t -\hat{x}_t\label{eq:global-1}\\
%     u_t &=  \clm{*u}{t}(0,\hat{w}_{t:t-T+1})\\
%     \hat{x}_{t} &=  \clm{*x}{t}(0,0,\hat{w}_{t-1:t-T+1})
% \end{align}
% \end{subequations}
% where $\{\CLM{*x}, \CLM{*u}\}$ denote the operators of the form \eqref{eq:NL-map}, with $\R{i}{}$, $\M{i}{}$ replaced by the solutions $\R{*i}{}$, $\M{*i}{}$ of the problem \eqref{eq:S2}.
% \begin{subequations}
% \begin{align}
% \label{eq:short-hand}
% \clm{*u}{t}(0,\hat{w}_{t:t-T+1})= \sum^{T-1}_{\tau = 0} &\M{*1}{\tau+1} \p1{\hat{w}_{t-\tau}} + \nonumber\\ &\M{*2}{\tau+1}(\p2{\hat{w}_{t-\tau}}-\p1{\hat{w}_{t-\tau}})\\
% \clm{*x}{t}(0,\hat{w}_{t:t-T+1}) = \sum^{T-1}_{\tau = 0} &\R{*1}{\tau+1}  \p1{\hat{w}_{t-\tau}} +\nonumber\\ 
% &\R{*2}{\tau+1}(\p2{\hat{w}_{t-\tau}}-\p1{\hat{w}_{t-\tau}})
% \end{align}\end{subequations}
% Note that we can freely choose $\eta_1$ as a hyperparameter. For the special case when $\eta_1$ is $0$, blending controller $\SL{\CLM{x}}{\CLM{u}}$ recovers linear \textit{safe} controller $\SL{\CLM{x,2}}{\CLM{u,2}}$ as the linear solution to \eqref{eq:const-lqr}. On the other hand, if $\eta_1$ fixed to be $(\eta_2-\epsilon)$, with $\epsilon$ arbitrarily small \footnote{This is to ensure \eqref{eq:safety-1} and \eqref{eq:safety-2} are well-defined.}, then constraints \eqref{eq:safety-1} and \eqref{eq:safety-2} could be arbitrarily relaxed, resulting in an arbitrary approximation to the performance controller $\SL{\CLM{x,1}}{\CLM{u,1}}$ as a solution to the unconstrained LQR problem. Therefore, $\eta_1$ serves as a tuning knob that balances the final blending controller to lie between pure performance-based strategy and the conservative safe strategy depending on whether estimated disturbance is small.
The next theorem states a main result of this paper: The synthesized controller $\SL{\CLM{*x}}{\CLM{*u}}$ from \eqref{eq:S2} outperforms any optimal linear controller for the constrained LQR problem.
\begin{thm}\label{thm:nlslsvssls}
For all $\eta_1 \in [0,\eta_2]$, the nonlinear system level controller $\SL{\CLM{*x}}{\CLM{*u}}$ achieves lower optimal LQR cost for \eqref{eq:const-lqr} than any linear solution to \eqref{eq:const-lqr}.
\end{thm}
\begin{proof}
First, recall that restricting $\b{K}$ to be linear in problem \eqref{eq:const-lqr} is equivalent to restricting $\CLM{x}$ and $\CLM{u}$ to be linear in the equivalent formulation \eqref{eq:const-lqrclm}. Furthermore, notice that under the restriction of linear $\{\CLM{x}, \CLM{u}\}$, problem \eqref{eq:const-lqrclm} is equivalent to \eqref{eq:S2} with the added constraint $\R1{} = \R2{}$, $\M1{}=\M2{}$, which proves that any solution $\{\CLM{*x}, \CLM{*u}\}$ of problem \eqref{eq:S2} achieve smaller cost than a linear solution $\{\CLM{x,lin*}, \CLM{u,lin*}\}$ of \eqref{eq:const-lqrclm}.
\end{proof}
%\begin{coro}\label{thm:n-nlslsvssls}
%The N-blend nonlinear system level controller $\SL{\CLM{x}}{\CLM{u}}$ of the form \eqref{eq:n-blend} constructed from the solution of \eqref{eq:S2} with \eqref{eq:safety-1} and \eqref{eq:safety-2} replaced with the following:
%\begin{subequations}
%\begin{align}
%&\sum_{i = 1}^N (\eta_i - \eta_{i-1})\|R^{(i)}\|_{\infty} \leq x_{max}\\
%&\sum_{i = 1}^N (\eta_i - \eta_{i-1})\|M^{(i)}\|_{\infty} \leq u_{max} 
% \end{align}
%\end{subequations}
%with  $\eta_{max} = \eta_N \geq\eta_{N-1} \geq \dots \geq \eta_0 =  0$
%achieves lower optimal LQR cost for \eqref{eq:const-lqr} than any linear solution to \eqref{eq:const-lqr}.
%\end{coro}
%\begin{proof}
%The same reasoning as \thmref{thm:nlslsvssls} applies.
%\end{proof}
\begin{coro}\label{thm:n-nlslsvssls}
	The N-blend nonlinear system level controller $\SL{\CLM{x}}{\CLM{u}}$ of the form \eqref{eq:n-blend} constructed from the solution of \eqref{eq:S2} for $N$ linear CLMs
	with  $\eta_{max} = \eta_N \geq\eta_{N-1} \geq \dots \geq \eta_0 =  0$
	achieves lower optimal LQR cost for \eqref{eq:const-lqr} than any linear solution to \eqref{eq:const-lqr}.
\end{coro}
\begin{proof}
	The same reasoning as the proof of \thmref{thm:nlslsvssls} applies.
\end{proof}


\subsection{Distributed Controller for Constrained LQR}
\label{sec:ls-lqr}
Thanks to the particular form of \eqref{eq:n-blend}, when the projection is chosen to be the saturation projection \defref{def:sat}, structural constraints of controller such as sparsity and delay constraints can be added in a convex way to the synthesis procedure described in \secref{sec:nlsls-take}. This is because imposing structural constraints on the nonlinear controller \eqref{eq:n-blend} is equivalent to imposing them on the linear CLM components of \eqref{eq:n-blend}. Detailed in \cite{anderson2019system}, localization of disturbance, communication and actuation delay, as well as sparsity pattern are all convex constraints in terms of linear CLMs in the linear System Level Synthesis framework. Specifically, all mentioned constraints could be cast as a convex subspace $\mathcal{S}_x$ and $\mathcal{S}_u$ for linear CLMs $\CLM{x,i}$,$\CLM{u,i}$,$i \in \set{N}$ in $\SL{\TU}{\TX}$. Therefore, the nonlinear controller synthesis in \secref{sec:nlsls-take} naturally inherits all capabilities of the linear system level controllers in terms of distributed controller syntehsis. 







==> nlsls_v1.tex <==
 This section will focus on introducing the notion of closed loop maps as causal operators w.r.t. a general nonlinear causal system. Moreover, we summarize necessary and sufficient conditions for operators to be closed loop maps and how they can be realized by a dynamic controller\cite{NLSLSHODoyle2019}.

\subsection{Closed Loop Maps of Nonlinear Systems}
Consider a general discrete-time nonlinear system with additive noise
\begin{align} \label{eq:sys}
x_{t+1} = f(x_{t},u_{t}) +w_t
\end{align}
where $x_t\in \mathbb{R}^n$, $u_t\in \mathbb{R}^p$, $w_t\in \mathbb{R}^n$ and $f:\RR^{n \times \N} \times \RR^{p \times \N} \rightarrow \RR^{n \times \N}$ is a causal operator with zero initial condition. Assume that $w_t$ can not be measured and that $u_t$ is generated by some $\b{K}:\RR^{n\times \N} \rightarrow \RR^{p \times \N}$, i.e. $\b{u} = \b{K}(\b{x})$:
\begin{align}\label{eq:u}
u_t = K_t\left(x_{t:0} \right)
\end{align}



% Furthermore let's make the following smoothness assumption:
%\begin{asp}\label{asp:lip}
%$f(x,u)$ is Lipshitz w.r.t $x$ and $u$ with the step $L$.
%\end{asp}
For a fixed disturbance sequence $\b{w}$, the dynamics \eqref{eq:sys} produces unique closed loop trajectories for state $\b{x}$ and input $\b{u}$. Therefore, given a fixed $\b{K}$, the dynamics induce a causal map from $\b{w}$ to $\b{x}$, $\b{u}$ and we will call the corresponding operators disturbance-to-state and disturbance-to-input \textit{closed loop maps}, respectively:
\begin{defn}[Closed Loop Maps]\label{def:clm}
We will call the operators $\b{\Phi}^{\b{w} \rightarrow \b{x}}_{[f,\b{K}]}:\RR^{n \times \N} \rightarrow \RR^{p \times \N}$ and $\b{\Phi}^{\b{w} \rightarrow \b{u}}_{[f,\b{K}]}:\RR^{n \times \N} \rightarrow \RR^{p \times \N}$ 
the disturbance-to-state and disturbance-to-input closed-loop maps(CLMs) of system $f$ w.r.t. controller $\b{K}$ if they map disturbance sequences $\b{w}$ to the corresponding state and input sequences $\b{x}$, $\b{u}$ of the system \eqref{eq:sys}, \textit{i.e.},
\begin{align}
&& x_{t+1} = f(x_{t},K_{t}(x_{t:0})) +w_t \\
&\Leftrightarrow &   \b{x} = \CLMofK{x}{\b{K}} (\b{w}), \quad \b{K}(\b{x}) = \CLMofK{u}{\b{K}}(\b{w})
\end{align}
we say the pair of operators $\{\CLM{x}$, $\CLM{u}\}$ is CLM of system \eqref{eq:sys}, if there exists a \textit{realizing} controller $\b{K}'$ such that
\begin{align}
&\CLM{x}=\CLMofK{x}{\b{K}'} &\CLM{u}=\CLMofK{u}{\b{K}'}
\end{align}
\end{defn}
The following theorem characterizes the space of CLMs for a given system $f$:
\begin{thm}\label{thm:sufnec}
$\CLM{x}$ and $\CLM{u}$ are CLMs of \eqref{eq:sys} if and only if they satisfy the following functional equations for all time $t$.
\begin{align}
\label{eq:feasnl}
\clm{x}{t}(w_{t:0}) &= \clm{x}{t}(0,0,w_{t-2:0}) + w_{t-1}\\
\label{eq:opfunceq_red}\clm{x}{t+1}(0,0,w_{t-1:0}) &= f(\clm{x}{t:0}(0,w_{t-1:0}),\clm{u}{t:0}(0,w_{t-1:0})) \nonumber
\end{align}
\end{thm}

%%%
\subsection{System Level Controllers}
We will call the realizing controllers of CLM pair $\{\CLM{x},\CLM{u}\}$ the \textit{System Level} (SL)-controllers
\begin{defn}[SL Controller]\label{def:SL}
Given causal operators $\TX:\RR^{n \times \N} \rightarrow \RR^{n \times \N}$, $\TU:\RR^{n \times \N}\rightarrow \RR^{p \times \N}$ define the system level(SL) controller as the operator $\b{K}(\b{x}): \RR^{n \times \N} \rightarrow \RR^{p \times \N}$ with realization
%\begin{align}
%u_t = K_t(x_{t:0}) = \Tu{t}(0,\hat{w}_{t:1})
%\end{align}
%where $\hat{w}_t$ is computed through the recursion
%\begin{subequations}
%\label{eq:SLeq}
%\begin{align}
%\hat{w}_0 &= x_0\\
%\hat{w}_1 &= x_1-\Tx{1}(0,0)\\
%&\dots \nonumber\\
%\hat{w}_t &= x_t-\Tx{t}(0,0,\hat{w}_{t-1:1})
%\end{align}
%\end{subequations}
\begin{subequations}
	\label{eq:SLeq}
	\begin{align}
	u_t = K_t(x_{t:0}) &= \Tu{t}(0,\hat{w}_{t:1})\\
	\hat{w}_0 &= x_0\\
	\hat{w}_t &= x_t-\Tx{t}(0,0,\hat{w}_{t-1:1})
	\end{align}
\end{subequations}
We will write $\b{K}=\SL{\TX}{\TU}$ to underscore that an operator $\b{K}$ is the system level (SL) controller of the CLMs $\{\TX$, $\TU\}$ and will refer to $\hat{w}_t$ as the internal state of $\b{K}$.
\end{defn}

% Given any system-level controller $\b{K}=\SL{\TX}{\TU}$, define $\b{x}'$, $\b{u}'$ as the input and output of the operator, \textit{i.e.}, $\b{u}' = \b{K}(\b{x}')$. Then the SL controller preserves the following important relation between $\b{u}'$, $\b{x}'$ and it's internal state $\hat{\b{w}}$:
% \begin{subequations}
% \begin{align}\label{eq:invSL}
%     x'_t &= \Tx{t}\left(0,0,\hat{w}_{t-1:1}\right)+\hat{w}_{t}\\
%     u'_t &= \Tu{t}\left(0,\hat{w}_{t:1}\right)
% \end{align}
% \end{subequations}

% Consider the closed loop of the nonlinear system \eqref{eq:sys} with the SL-controller $u_t = K_t(x_{t:0}+v_{t:0})+d_t$ subject to bounded perturbations $\b{v}$ and $\b{d}$ in state and input. Using the above relation, the dynamics of the closed loop can be written as:
% \begin{subequations}
% \label{eq:cleq}\begin{align}
%   \label{eq:clint} \hat{w}_{t+1} &= \Delta_t(\hat{w}_{t:1},v_t,d_t) + w_t\\
%     \label{eq:clx}     x_t &= \Tx{t}\left(0,0,\hat{w}_{t-1:1}\right)+\hat{w}_{t}-v_t\\
%     \label{eq:clu}u_t &= \Tu{t}\left(0,\hat{w}_{t:1}\right)+d_t
% \end{align}
% \end{subequations}
% where $\b{\Delta}$ stands for the operator:
% \begin{align}
%     \notag \Delta_t(&\hat{w}_{t:1},v_t,d_t):= f(\Tx{t:0}(0,\hat{w}_{t:1})-v_t, \\
%     \label{eq:Delta} &\Tu{t:0}(0,\hat{w}_{t:1})+d_t) - \Tx{t+1}\left(0,0,\hat{w}_{t:1}\right)
% \end{align}


% \begin{thm}[Realizing Controller of CLMs\cite{NLSLSHODoyle2019}]\label{thm:real}
% \phantom{as} Consider the dynamics \eqref{eq:cleq} of the system \eqref{eq:sys} in closed loop with an SL-controller $\b{K} = \SL{\CLM{x}}{\CLM{u}}$. Then, if $\CLM{x}$ and $\CLM{u}$ are CLMs of \eqref{eq:sys}, then $\CLMofK{x}{\b{K}} = \CLM{x}$ and $\CLMofK{u}{\b{K}} = \CLM{u}$.
%  \end{thm}
 \begin{thm}[Stability of Closed Loop\cite{NLSLSHODoyle2019}]\label{thm:stability}
If $f$ is uniformly continuous and the operators $\CLM{x},\CLM{u}$  are $\ell_p$-stable CLMs of \eqref{eq:sys} (or $\ell_p$ finite gain-stable), then the closed loop dynamics are $\ell_p$-stable (or finite gain $\ell_p$-stable) w.r.t to the bounded perturbations $\b{w}$, $\b{d}$ and $\b{v}$. 
% Moreover, if $\CLM{x},\CLM{u}$ are \textit{not} CLMs of the system \eqref{eq:sys}, then the previous stability guarantee still holds true if and only if the internal dynamics \label{eq:clint} are $\ell_p$-stable/finite gain $\ell_p$-stable. 
\end{thm}
%
%A particular subclass of stable operators that we will consider in this work are operators of finite memory, which are defined as follows:
%\begin{defn}[CLM with Finite Memory]\label{def:FM}
%CLM $\{\CLM{x},\CLM{u}\}$ are said to have finite memory of horizon $T$ if
%\begin{equation}
%    \clm{x}{t+1}(0,w_{t:0}) =
%    \begin{cases}
%    \clm{x}{t+1}(0,w_{t:0}) & \forall t < T \\
%        \clm{x}{t+1}(0,w_{t:t+1-T},0,\dots,0) & \forall t \geq T
%    \end{cases}
%\end{equation}
%
%\end{defn}
\subsection{Relation to Linear System Level Approach}
If we restrict the previous analysis to linear time-invariant (LTI) systems and controllers, we recover the results of \cite{anderson2019system} for the state-feedback case.
If $x_{t+1} = Ax_t + Bu_t + w_t$ and $\b{K}$ is a LTI operator, then the corresponding linear closed loop maps are LTI as well.
%With the abbreviation $\CLM{x} = \CLMofK{x}{\b{K}}$, $\CLM{u} = \CLMofK{x}{\b{K}}$, the CLM takes the realization
In this case, the CLMs take the realization
\begin{subequations}
\label{eq:linear-maps}
\begin{align}
    \clm{x}{t}(0,w_{t-1:0}) & = \sum^{t}_{k=1}R_k w_{t-k}\\
    \clm{x}{u}(0,w_{t-1:0}) & = \sum^{t}_{k=1}M_k w_{t-k}
\end{align}
\end{subequations}
where $R_k \in \RR^{n \times n}$, $M_k \in \RR^{p \times n}$ are called associated matrices of $\CLM{x}$ and $\CLM{u}$. Moreover, the corresponding CLM feasibility condition reduces to the affine constraint on the matrices $R_k$, $M_k$ which coincides with the linear System Level Synthesis(SLS) feasibility conditions derived in \cite{anderson2019system}. Let $\CLM{x}$ and $\CLM{u}$ be further constrained to have Finite Impulse Response (FIR) of horizon $T$, then parameterization of the CLMs in \eqref{eq:feasnl}  reduces to:
\begin{subequations}
\label{eq:lin-feaibility}
\begin{align}
    &R_{1} = I \\
    &R_{k+1} = A R_k + B M_k \\
    &A R_{T-1} + B M_{T-1} = 0
\end{align}
\end{subequations}
 Similarly, a strictly causal system level controller $\b{K} = \SL{\CLM{x}}{\CLM{u}}$ in \eqref{eq:SLeq} with LTI operators $\CLM{x}$, $\CLM{u}$ satisfying the above becomes 
\begin{align}
\hat{w}_t &= x_t - \sum^{\min\{t,T-1\}}_{k=1}R_{k+1}\hat{w}_{t-k}\\
\label{eq:nl-controller-2} u_t &=   \sum^{\min\{t,T-1\}}_{k=0}M_{k+1}\hat{w}_{t-k}
\end{align}
which describes the standard SLS controller in \cite{anderson2019system}. Since the CLMs are chosen to be FIR, internal stability of the closed-loop system is immediate.

% since by definition of CLMs, we have the following closed-loop behaviour:
%\begin{align}
%\label{eq:lin-controller}
%&x_{t} = \sum^{\min\{t,T\}}_{k=1}R_{k}w_{t-k},
%&u_{t} = \sum^{\min\{t,T\}}_{k=1}M_{k}w_{t-k}
%\end{align} 
%Recall from \cite{slsacc}, that linear CLMs $\CLM{x}$, $\CLM{u}$ are called finite impulse response(FIR) CLM of horizon $T$, if $R_T$, $M_T$ satisfy $$. The corresponding closed loop is then trivially stable since the closed loop has a finite impulse response and enforces the following CLM between the disturbance $\b{w}$ and $\b{x}$, $\b{u}$: 



==> prelim_v1.tex <==
%We will use the following abbreviation whenever it will be cumbersome to write expressions with functions of many arguments: Define $f(x_{i:j})$ to be $f(x_{i},x_{i+1},\dots, x_{j})$ for ($i <j$) and $f(x_{i},x_{i-1},\dots, x_{j})$ for ($i >j$), respectively.  Unless otherwise specified, $||\cdot||$ denotes the infinity norm for vectors and induced infinity norm for matrices. 

 We will define  $\mathbb{R}^{n \times \mathbb{N}}$ to be spaces of sequences of vectors in $\RR^n$. A causal operator will be denoted in bold capital letters $\b{T}$ and will represent maps of the form $\RR^{n \times \N} \rightarrow \RR^{k \times \N}$.The corresponding functions that map $x_{t:0}$ to $(\b{T}(\b{x}))_t$ are denoted as $T_t:\RR^{n \times (t+1)} \rightarrow \RR^k $ and the realization of a causal operator is $\b{T}(\b{x})=(T_0(x_0), T_1(x_1,x_0),T_2(x_2,x_1,x_0), \dots)$.
% Denote column-wise concatenation through $\left[A;B \right] := \left[A^T,B^T\right]^T$.
 Sequences of vectors $(x_t)^{\infty}_{t=0}$ will be denoted by small bold letters $\b{x}$ unless otherwise specified and $\b{x}_t$ is the vector $x_t$ at $t$th time step in the sequence with $x^j_t$ denotes the $j$th element of vector $x_t$. We will use the notation $x_{i:j}$ to refer to the truncation of the sequence $[x_{i},x_{i+1},\dots, x_{j}]$. 
%  The transpose of truncated sequence of vectors is $x_{1:k}^T := [x_1^T,x_2^T,\dots, x_k^T]^T$.  
 Furthermore, we will adopt $\|.\|_{p}$ to refer to the $\ell _p$ norm and induced norm on vectors and matrices. The set of positive integers ranging from 1 to $N$ will be denoted as $\set{N}$.
% \begin{align}
% \ell^{n}_{p} &:= \left\{\b{x} \in \mathbb{R}^{n \times \mathbb{N}} \left| \Nxy{\b{s}}{p} < \infty, \quad s_k := \Nxy{x_k}{} \right. \right\} \\
% \Nxy{\b{x}}{p} & := \Nxy{(\Nxy{x_0}{},\Nxy{x_1}{},\dots)}{p}
% \end{align}
% In particular, $\ell^{n}_{\infty}$ denotes the space of all bounded sequences in the normed vector space $(\Nxy{.}{},\RR^n)$. 
%\subsection{Causal Operators}
% Operators will be denoted in bold capital letters $\b{T}$ and will represent maps of the form $\RR^{n \times \N} \rightarrow \RR^{k \times \N}$. An operator will be called causal if $(\b{T}(\b{x}))_t$ depends only on $x_{t:0}$. The corresponding functions that map $x_{t:0}$ to $(\b{T}(\b{x}))_t$ are denoted as $T_t:\RR^{n \times (t+1)} \rightarrow \RR^k $ and the realization of a causal operator is $\b{T}(\b{x})=(T_0(x_0), T_1(x_1,x_0),T_2(x_2,x_1,x_0), \dots)$.
% 
% \begin{defn}[ Stable Causal Operators]
%A causal operator $\b{T}:\RR^{n \times \N} \rightarrow \RR^{k \times \N}$ is defined to be $\ell_p$-stable if $\Nxy{\b{x}}{p} < \infty $ implies $\Nxy{\b{T}(\b{x})}{p} < \infty$ and \textit{finite gain} $\ell_p$-stable with gain $\gamma \geq 0$ if there exist $\beta \geq 0$  such that $\Nxy{\b{T}(\b{x})}{p} \leq  \gamma\Nxy{\b{x}}{p} + \beta $ for all $\b{x} \in \ell^n_p$.
%\end{defn}

% \begin{defn}[Causal Operator]\label{def:caus}
%  An operator $\b{T}:\RR^{n \times \N} \rightarrow \RR^{k \times \N}$ is \textit{causal}, if there exist functions $T_t:\RR^{n \times (t+1)} \rightarrow \RR^k$ such that $(\b{T}(\b{x}))_t = T_t(x_{t:0})$ for all $t$ and sequences $\b{x} \in \RR^{n \times \N}$. If in addition $T_t(x_{t:0}) = T_t(0,x_{t-1:0}) $ holds $\b{T}$ is called \textit{strictly causal}. Furthermore, let $T_{i:j}: \RR^{n \times (\max\{i,j\}+1)} \rightarrow \RR^{k \times (|j-i|+1)}$ be the truncation map defined as:
% \begin{align}
% T_{i:j}(x_{j:0}) &:= (\b{T}(\b{x}))_{i:j} \quad \text{for }j\geq i \\
% T_{i:j}(x_{i:0}) &:= (\b{T}(\b{x}))_{i:j} \quad \text{for }j<i.
% \end{align}
% \end{defn} 

%New Stuff
%%%%

==> scalar_v1.tex <==
In this section, we will show that the simple projection nonlinearity in \eqref{eq:NL-map} gives the proposed nonlinear blending controller $\SL{\CLM{x}}{\CLM{u}}$  discussed in \secref{sec:blend} a natural anti-windup property. 
%In particular, it will be illustrated that $\SL{\CLM{x}}{\CLM{u}}$   recovers simple anti-windup schemes for integrator windup problem under input saturation. 
We choose a scalar case to start the analysis for ease of exposition.

Consider the following \textit{linear} controller design problem:
\begin{subequations}
\label{eq:scalar}
\begin{align}
\label{eq:costsls}\min_{\b{K}} &  \lim_{T \rightarrow \infty}\frac1T\sum_{k = 0}^{T} x^2 \\
s.t.\,\,\,\,\,\,\,\,\,  x_{t+1} &= x_{t} + u_t + w_t, \quad x_0 = 0\\
 u_t &= \b{K}(x_{t:0})\\
 \b{w} = \b{1}: \,\,\, x_t &= 0 \quad \forall t \geq 2   \label{eq:rpa}
\end{align}
\end{subequations}
The performance objective \eqref{eq:rpa} states that the system should return to origin within two time steps after a step disturbance hits. Such objective could only be fulfilled when the controller has an internal integrator where step disturbance can be perfectly rejected.

One can check that the optimal \textit{integral} SL-controller for \eqref{eq:scalar} is 
\begin{subequations}
\label{eq:rpa-controller}
\begin{align}
    \hat{w}_{t+1} &= \hat{w}_t +x_t\\
    u_t &= -x_t - \hat{w}_t
\end{align}
\end{subequations}
Because integral action is required to perfectly reject step input, input saturation could cause severe windup behaviour leading to instability. As shown in \figref{fig:scalar}, bounded sequence of disturbance between $-1$ and $1$ causes severe windup effects for integrator controller \eqref{eq:rpa-controller} under saturation: $\text{sat}(u_t) = \text{sign}(u_t)\min\{|u_t|,1\}$. 
The simplest strategy one could adopt in this case is to switch to a controller synthesized from \eqref{eq:scalar} without performance requirement \eqref{eq:rpa} in the face of saturation to ensure closed loop stability. Inspection of \eqref{eq:scalar} verifies the optimal \textit{non-integral} SL-controller is simply a deadbeat controller 
\begin{equation}
\label{eq:nonrpa-controller}
    u_t = -x_t
\end{equation}
% The simplest strategy one could adopt in this case is to "turn off" the integrator part of the controller, \textit{i.e.}, switching to $G_{aw}(z) = -2$ in the face of saturation to ensure closed loop stability. 
However, the non-integral controller does not satisfy the performance objective of step input rejection. Therefore, one naturally seeks a "middle ground" between \eqref{eq:rpa-controller} and \eqref{eq:nonrpa-controller} where under small signals, integral actions are taken to meet performance objective while guaranteeing stability under large signals.
\begin{figure}[h]
 \centering
 \includegraphics{scalar.pdf}
 \caption{Saturating response to large worst-case disturbance for the integral controller (dotted-red), anti-windup controller (blue), and naive blending controller (green): Integral controller becomes unstable in the face of input saturation. The response of simple anti-windup schemes that simply turn off the integral portion of the controller is recovered by the proposed naive blending controller.}
 \label{fig:scalar}
% \end{figure}

% \begin{figure}[h]
%  \centering
 \vspace{0.00cm}
 \includegraphics{scalar-db-vs-blend.pdf}
 \caption{Response of Simple Linear Anti-windup Controller (blue) VS. Proposed Blending (green) for small step Input: The simple linear anti-windup controller used globally ensures stability under saturation at the cost of forfeiting the step response performance objective. The naive blending controller recovers this performance objective in the case of small steps while still ensure stability under saturation.}
 \label{fig:db-vs-blend}
\end{figure}
Consider now the blending nonlinear controller $\SL{\CLM{x}}{\CLM{u}}$ from \eqref{eq:NL-map}. A naive scheme is simply blending the \textit{integral} and \textit{non-integral} controller with a small $\eta_1$ value. Denote the transformed controller internal state $\tilde{w}_t = \p{1}{\hat{w}_t}$, the resulting blending nonlinear SL-controller is:
\begin{subequations}
\label{eq:scala-blend}
\begin{align}
    \tilde{w}_{t+1} &= \p{1}{\tilde{w}_t + x_t}\\
    u_t &= -x_t-\tilde{w}_t
\end{align}
\end{subequations}
It is now clear that the projection nonlinearity in \eqref{eq:NL-map} offers a natural anti-windup property since the essence of traditional anti-windup schemes \cite{kothare1994unified} is to stop the integrator from accumulating errors. As demonstrated in \figref{fig:scalar} and \figref{fig:db-vs-blend}, the blending controller achieves similar stable behaviour as the non-integrator controller under controller saturation but recovers performance in the small-signal regime. 

For this scalar example, the projection nonlinearity of \eqref{eq:NL-map} automatically allow the naive blending scheme to have anti-windup property while preserving performance under small disturbance. Despite the simplicity of the projection nonlinearity in \eqref{eq:NL-map}, we will see in the next section that the anti-windup property for the naive blending scheme extends to the large-scale case.

==> simulation_v1.tex <==
\subsection{Constrained LQR}
To corroborate the results presented in the previous sections, we demonstrate the performance of a four-zone nonlinear blending controller with radial projection compared against the optimal linear controller for the constrained LQR problem of an open-loop unstable system: 
\begin{align}
    x_{k+1} &= \begin{bmatrix}1&1&0\\1&2&1\\0&1&1 \end{bmatrix}x_k + \begin{bmatrix}0\\0\\1 \end{bmatrix}u_k +w_k
\end{align}
with $u_{max} = 40$, $x_{max} = 15$, $\eta_{max} = 1$, $Q = I_3$, $P = 10$. The disturbances $w_k$ are chosen to be a truncated i.i.d. gaussian random variables with variance $\sigma^2$. \figref{fig:performance} shows the optimal cost improvement of the presented nonlinear approach over the optimal linear controller for different choices of variance $\sigma^2$. \figref{fig:performance} showcases that the proposed controller can exploit the knowledge of the disturbance distribution to achieve performance improvement over the linear optimal linear controller: For small $\sigma$ the proposed controller gains more than 30\% cost reduction over safe controller. On the other hand, with increasing $\sigma$, large disturbances in the system become more likely, and therefore the opportunity to improve upon the linear optimal controller is reduced.
\begin{figure}[h]
 \centering
 \includegraphics[scale = 0.75]{figure/performance_1.pdf}
 \caption{Performance improvement of optimal nonlinear controller $\SL{\CLM{*x}}{\CLM{*u}}$ over optimal linear controller $\SL{\CLM{x,lin*}}{\CLM{u,lin*}}$ for different variances $\sigma^2$ of the non-truncated disturbance. The nonlinear blending controller synthesizes over 4 linear controllers w.r.t. to the projection parameters $\eta_1= 0.05, \eta_2 = 0.1, \eta_3 = 0.2, \eta_4 = \eta_{max} = 1 $}
 \label{fig:performance}
\end{figure}

\subsection{Distributed Anti-Windup Controller}
Consider a bi-directional chain system with $i$th node's dynamics being
\begin{equation}
\label{eqn:sim}
    x^i_{t+1} = (1- 0.4\lvert \mathcal{N}(i) \rvert  ) x^i_t + 0.4 \sum_{j \in \mathcal{N}_i} x^j_t + \sat(u^i_t,u_{max}) + w_t^i \nonumber
\end{equation}
where $\mathcal{N}(i)$ denotes the set of vertices that has an edge connected to $i$th vertex and $w_t^i$ is the $i$th coordinate of disturbance vector at time $t$. In particular, $\|\b{w}\|_{\infty}\leq 1$ and $x_0 = 0$.  One can check that the overall chain system is open-loop marginally stable.

We illustrate the anti-windup property of the nonlinear controller \eqref{eq:n-blend} in the decentralized setting with additional sparsity, locality, and delay constraints. First, a nominal integral controller for this system is designed and dubbed as the \textit{Integral Controller}. Due to its integral structure, the \textit{Integral Controller} for the unconstrained closed loop guarantees convergence of the state to the origin under persistent disturbance, \textit{i.e}, step rejection. In comparison, a second linear controller synthesized from standard constrained LQR problem that guarantees stability for all admissible $\b{w}$ under saturation is generated. We refer to this linear controller as the \textit{Non-integral Controller} since the states only stay bounded under persistent admissable disturbance.  

 The nonlinear controller with saturation projection here is chosen to be a two-zone blending controller consisted of CLMs of the form \eqref{eq:NL-map}. The simulation shows the anti-windup property as well as preservation of step rejection in both large- and small-disturbance schemes of the proposed method. \figref{fig:ls-worst} shows that the blending controller stabilizes the system while integral controller becomes unstable under worst-case bounded disturbance. On the other hand, the proposed blending controller preserves performance of step rejection while the linear Non-integral Controllers forfeits the performance objective in order to preserve stability in the saturated closed loop. In this chain example, we allow 1 time step communication delay between nodes and actuation delay with 50\% control authority. The localization pattern imposed on the system response allows $\SL{\CLM{x}}{ \CLM{u}}$ to be implemented in local patches, therefore making the controller distributed.
% \begin{equation}
% \label{eqn:sim}
%     x^i_{t+1} = \rho (1-\lvert \mathcal{N}(i) \rvert \alpha ) x^i_t + \rho \alpha \sum_{j \in \mathcal{N}_i} x^j_t + u^i_t
% \end{equation}




\begin{figure*}
\centering
%   \subfigure[Integral Controller under Worst-case Disturbance/under Staggered Step Disturbance]{ \includegraphics[scale = 0.5, trim = 5cm 7.8cm 6cm 7.8cm, clip]{worst-rpa.pdf}}
 \subfigure[Integral Controller]{ \includegraphics{figure/worst-rpa.pdf}}
%  \caption{Response of Integral Controller}
  \subfigure[Non-integral Controller]{ \includegraphics{figure/worst-nonrpa.pdf}\label{fig:ls-act}}
    \subfigure[Nonlinear Blending Controller ]{ \includegraphics{figure/worst-blend.pdf}\label{fig:ls-act}}
     % \subfigure[Integral Controller ]{ \includegraphics[scale = 0.48, trim = 5cm 8.5cm 6cm 8.5cm, clip]{step-rpa.pdf}}
     \subfigure[Integral Controller ]{ \includegraphics{figure/step-rpa.pdf}}   
%  \caption{Response of Integral Controller}
  \subfigure[Non-integral Controller ]{ \includegraphics{figure/step-nonrpa.pdf}\label{fig:ls-act}}
    \subfigure[Nonlinear Blending Controller ]{ \includegraphics{figure/step-blend.pdf}\label{fig:ls-act}}
   \caption{\textit{\textbf{Worst-case (top row) and Staggered Step Input (bottom row) Response} under Saturation for a marginally stable 20-node Chain System with Sparse Actuation}: \textit{Top Row}: Worst-case disturbance propagates through space-time for the saturated chain system. The nonlinear controller possesses the anti-windup property of the non-integral controller. In addition to  anti-windup, the proposed controller is localized and accommodates sparse actuation, communication delay, and controller sparsity constraints. Here every other node has a control input (50\% actuation) with 1 time step actuation delay and 1 time step communication delay between nodes, while enforcing a controller sparsity that conforms to the communication pattern of dynamics matrix $A$. \textit{Bottom Row}: Response to small step disturbances at node 8,10,12 entering at time 2,6,10, respectively.The blending controller not only stabilizes under saturation but also recovers the performance objective of rejecting small step disturbances. 
}
   \label{fig:ls-worst}
\end{figure*} 

%Worst-case (top row) and Staggered Step Input (bottom row) Response} under Saturation for a marginally stable 20-node Chain System with Sparse Actuation}: \textit{Top Row}: The heatmaps show how a worst-case disturbance is propagated through space-time for the saturated chain system. The integral controller becomes unstable due to saturation and the nonlinear controller possesses the anti-windup property of the non-integral controller.
%In addition to  anti-windup, the proposed controller is localized and accommodates sparse actuation, communication delay, and controller sparsity constraints. Here every other node has a control input (50\% actuation) with 1 time step actuation delay and 1 time step communication delay between nodes, while enforcing a controller sparsity that conforms to the communication pattern of dynamics matrix $A$. \textit{Bottom Row}: Response to small step disturbances at node 8,10,12 entering at time 2,6,10, respectively.The proposed blending controller not only stabilizes under saturation but also recovers the performance objective of rejecting small step disturbances. This contrasts against the non-integral controller, which sacrifices small-signal performance for stability. 


==> windup_v1.tex <==
 We have showed  that projection nonlinearity of the controller \eqref{eq:NL-map} provides simple and effective solution to the constrained LQR problem when disturbance is known to be bounded. Now consider a linear input saturated system where the disturbances and initial condition are not necessarily constrained to have a known norm bound:
\begin{align}
\label{eq:lin-sat}
x_{t+1} = Ax_t+ \sat(u_t,u_{max}) + w_t
\end{align}
where the saturation nonlinearity is applied element-wise to the vector $u_t$.
In this scenario, controller $\SL{\CLM{x}}{\CLM{u}}$ previously constructed with \eqref{eq:NL-map} \textit{no longer} realizes the designed CLMs \eqref{eq:NL-map} for \eqref{eq:lin-sat}. Rather, the internal dynamics of \eqref{eq:lin-sat} with $\SL{\CLM{x}}{\CLM{u}}$ can be checked to be:
\begin{align}
\label{internal}
\hat{w}_t = A(\hat{w}_{t-1}-\p{max}{\hat{w}_{t-1}}) + w_{t-1}
\end{align}
 Nevertheless, we would like the saturated system to degrade gracefully and preserve stability. Such property is traditionally achieved via anti-windup design\cite{hu2008anti}. Here, we show that the proposed nonlinear controller achieves natural anti-windup property. 
\begin{lem}
If $A$ is schur, then internal dynamics \eqref{internal} is BIBO-stable. Further, if $\|A\|_{p} < \lambda <1 $, then $\limsup_{t \rightarrow \infty} \|\hat{w}_t\|_{p} < \frac{1}{1-\lambda} \|\b{w}\|_{p}$ with $p \in \{1,\infty\}$
\end{lem}
\begin{proof} Omitted in the interests of space
	\end{proof}
Similar to the large-scale constrained LQR case, since the "anti-windup" controller for the saturated linear system \eqref{eq:lin-sat} is composed of linear CLMs synthesized from \eqref{eq:S2} without the state constraint \eqref{eq:safety-1}, as will be illustrated in \secref{sec:sim}, distributed controller constraints can be easily incorporated. Thus, the given nonlinear controller can be considered as a distributed anti-windup controller. 


%
%
%\subsection{old version}
%Thus far, we have shown
%
%
%A related and natural question to ask is whether such control strategy works for saturated systems. It is plausible that the projection nonlinearity provides natural anti-windup property where finite-gain stability of the closed-loop is preserved and the system recovers linear scheme quickly under saturation. Further, if the controller is anti-windup, will the distributed properties discussed in \secref{sec:ls-lqr}? The answers to these questions are affirmative.\todo[inline]{the last two sentences are weird, needs rephrasing} Since our framework seeks explicit operators that map disturbance to states, the following is immediate.
%\begin{lem}
%\label{lem:finite-gain}
%Given a linear system with actuation saturation that has zero initial condition, \textit{i.e}, $x_0 = 0$:
%\begin{align}
%\label{eq:lin-sat}
%    x_{k+1} = Ax_k + \text{sat}_{u_{max}}(u_k) + w_k
%    \end{align}
% and a bound on disturbance such that $\|\b{w}\|_{\infty} \leq \eta_{max}$, 
%the closed loop under a controller of the form \eqref{eq:n-blend} with saturation projection constructed from CLMs synthesized in \eqref{eq:S2} without state constraints has finite-gain stability for all admissible $\b{w}$:
%$$\|\b{x}\| \leq \gamma \|\b{w}\|$$
%where $\gamma = \sum_{i = 1}^N (\eta_i - \eta_{i-1})\|R^{(i)}\|$
%\end{lem}
%\todo[inline]{Should be inf-norm, right?}
%\begin{proof}
%Application of norm submultiplicativity gives the finite gain bound.
%\end{proof}
%
%\begin{lem}\label{thm:antiwinduplqr}
%Consider the same conditions in \lemref{lem:finite-gain}, if $A$ is schur, then there exists $\gamma >0$ such that for all $\b{w}\in \ell_{2}$, 
%$$\|\b{x}\|_{2} \leq \gamma \|\b{w}\|_{}.$$
%\end{lem}
%\begin{proof}
%Omitted in the interest of space.
%\end{proof}
%\todo[inline]{Do you require also $\|w\|_{\infty} \leq \eta_{max} $? you said same conditions.. also norms are missing }
%
%% \begin{thm}\label{thm:antiwinduplqr}
%%  Assume that $\SL{\CLM{*x}}{\CLM{*u}}$ is applied to the linear system with input saturation  of the form $$x_{k+1} = Ax_k + \text{sat}_{u_{max}}(u_k) + w_k.$$
%% Then, if $A$ is marginally stable, then $\b{x}$ and $\b{u}$ are bounded for any bounded $\b{w}$.
%% \end{thm}
%% \begin{proof}
%% Omitted in the interest of space.
%% \end{proof}
%


